Geometric Neural Process Fields

This paper addresses the challenge of Neural Field (NeF) generalization, where models must efficiently adapt to new signals given only a few observations. To tackle this, we propose Geometric Neural Process Fields (G-NPF), a probabilistic framework for neural radiance fields that explicitly captures uncertainty. We formulate NeF generalization as a probabilistic problem, enabling direct inference of NeF function distributions from limited context observations. To incorporate structural inductive biases, we introduce a set of geometric bases that encode spatial structure and facilitate the inference of NeF function distributions. Building on these bases, we design a hierarchical latent variable model, allowing G-NPF to integrate structural information across multiple spatial levels and effectively parameterize INR functions. This hierarchical approach improves generalization to novel scenes and unseen signals. Experiments on novel-view synthesis for 3D scenes, as well as 2D image and 1D signal regression, demonstrate the effectiveness of our method in capturing uncertainty and leveraging structural information for improved generalization.

==> Sections/3.2method.tex <==

% \js{Double check connection sentences between subsections}

\noindent \textbf{Notations.}
%We work on the 3D space.
% We denote 3D world coordinates with ${\bf{p}}=(x,y,z)$, and the camera viewing direction with $v=(\theta,\phi)$. 
% %from any 3D point in space with the angles $v=(\theta,\phi)$. %denoting pitch and yaw.
% The points in the 3D space have color $c^{{\bf{p}}, v}$ that depends on the 3D location $p$ and the viewpoint of the camera $\bf{v}$.
% The points also have a density value $\sigma^p$ that encodes how opaque that point is.
% We couple them together in $\bf{y}^p=\{c^{{\mathbf{p}}, v}, \sigma^p\}$.
% When examining a whole 3D object from multiple 3D locations in space, $i=1,...,N$, we denote the set of all 3D locations with $\mathbf{X}=\{\mathbf{x}^n\}_{n=1}^N$, and $\mathbf{Y}=\{\mathbf{y}^n\}_{n=1}^N$.
% Assuming a ray $r=(p, v)$ starting from location $p$ and from viewpoint $v$, with $x^r=\{x^r_i\}_{i=1}^P$ and $y^r=\{y^r_i\}_{i=1}^P$ we denote all the 3D locations, and colors on $P$ points sampled from the ray.
% Further, with ${\tilde{\bf{X}}}$ and ${\tilde{\bf{Y}}}$ we denote the observations we have, the set of camera rays ${\tilde{\bf{X}}} = \{  
% \tilde{\bf{x}}_n = r_n \}_n^{N}$, and the projected 2D pixels from the rays ${\tilde{\bf{Y}}} = \{  
% \tilde{\bf{y}}_n^p \}_n^{N}$. 
%
We denote 3D world coordinates by \(\mathbf{p} = (x, y, z)\) and a camera viewing direction by \(\mathbf{d} = (\theta, \phi)\). Each point in 3D space have its color \(\mathbf{c}(\mathbf{p}, \mathbf{d})\), which depends on the location \(\mathbf{p}\) and viewing direction \(\mathbf{d}\). Points also have a density value \(\sigma(\mathbf{p})\) that encodes opacity. We represent coordinates and view direction together as $\mathbf{x} = \{\mathbf{p},\mathbf{d} \}$, color and density together as \(\mathbf{y}(\mathbf{p}, \mathbf{d}) = \{\mathbf{c}(\mathbf{p}, \mathbf{d}), \sigma(\mathbf{p})\}\).
\str{This sentence sounds a bit strange, we can denote all 3D points like that anyways, no need to observe them from 'multiple locations', no? In general, I think the paragraph can be written more cleanly.}
When observing a 3D object from multiple locations, we denote all 3D points as \(\mathbf{X} = \{\mathbf{x}_n \}_{n=1}^N\) and their colors and densities as \(\mathbf{Y} = \{\mathbf{y}_n\}_{n=1}^N\).
Assuming a ray \(\mathbf{r} = (\mathbf{o}, \mathbf{d})\) starting from the camera origin \(\mathbf{o}\) and along direction \(\mathbf{d}\), we sample $P$ points along the ray, with \(\mathbf{x}^{\mathbf{r}} = \{{x}_i^\mathbf{r}\}_{i=1}^P\) and corresponding colors and densities \(\mathbf{y}^{\mathbf{r}} = \{{y}_i^{\mathbf{r}}\}_{i=1}^P\). Further, we denote the observations \(\widetilde{\mathbf{X}}\) and \(\widetilde{\mathbf{Y}}\) as: the set of camera rays \(\widetilde{\mathbf{X}} = \{\widetilde{\mathbf{x}}_n = \mathbf{r}_n\}_{n=1}^N\) and the projected 2D pixels from the rays \(\widetilde{\mathbf{Y}} = \{\widetilde{\mathbf{y}}_n\}_{n=1}^N\).



% \begin{figure}[t]
%   \centering
%   \includegraphics[width=0.49\textwidth]{Figures/problemstate.pdf} % Adjust the size and filename as needed
%   \caption{Framework.} % Caption for the figure
%   \label{fig:problem}
% \end{figure}



% \str{Can you clarify what exactly each notation style corresponds to? What is the $\sim$ for instance? The sampled new pixel views? And no tilde are the actual observations?}

\begin{figure}[htbp]
%\vspace{-5mm}
\centering
\centerline{
\includegraphics[width=0.95\columnwidth]{Figures/problemstate.pdf} 
} 
%\vspace{-2mm}
\caption{\textbf{Complete rendering from 3D points to a 2D pixel.}
}
%\vspace{-4mm}
\label{fig:problem}
\end{figure}

\textbf{Background on Neural Radiance Fields.}
We formally describe Neural Radiance Field (NeRF)~\citep{mildenhall2021nerf, arandjelovic2021nerf} as a continuous function \( f_{\text{NeRF}}: \mathbf{x} \mapsto \mathbf{y} \), which maps 3D world coordinates \(\mathbf{p}\) and viewing directions \(\mathbf{d}\) to color and density values \(\mathbf{y}\). 
That is, a NeRF function, \( f_{\text{NeRF}} \), is a neural network-based function that represents the whole 3D object (e.g., a car in Fig.~\ref{fig:problem}) as coordinates to color and density mappings. Learning a NeRF function of a 3D object is an inverse problem where we only have indirect observations of arbitrary 2D views of the 3D object, and we want to infer the entire 3D object's geometry and appearance.
With the NeRF function, given any camera pose, we can render a view on the corresponding 2D image plane by marching rays and using the corresponding colors and densities at the 3D points along the rays. Specifically, given a set of rays \(\mathbf{r}\) with view directions \(\mathbf{d}\), we obtain a corresponding 2D image. The integration along each ray corresponds to a specific pixel on the 2D image using the volume rendering technique described in~\cite{kajiya1984ray}, which is also illustrated in Fig.~\ref{fig:problem}. Details about the integration are given in Appendix~\ref{supp:nerf-render}. 



%\str{Write down the integral.}
%


% Neural Fields are normally considered as an optimization routine in a deterministic setting, whereby95
% the function fNeRF is fit perfectly to the available observations (akin to “overfitting” training data).


\subsection{Probabilistic NeRF Generalization}
% \js{probabilistic NeRF is not new}

\paragraph{Deterministic Neural Radiance Fields} Neural Radiance Fields are normally considered as an optimization routine in a deterministic setting~\citep{mildenhall2021nerf,barron2021mip}, whereby the function $f_{\text{NeRF}}$ fits specifically to the available observations (akin to ``overfitting'' training data).

\paragraph{Probabilistic Neural Radiance Fields} As we are not just interested in fitting a single and specific 3D object but want to learn how to infer the Neural Radiance Field of any 3D object,  we focus on probabilistic Neural Radiance Fields with the following factorization:
%
% \begin{equation}
%     p({\bf{\widetilde{y}}}|{\bf{\widetilde{x}}}, f_{NeRF}) \propto
%     \underbrace{p({\bf{\widetilde{y}}}| {\bf{{y}}}^{1:P}, {\bf{{x}}}^{1:P})}_{\text{Integration}}
%     \underbrace{p({\bf{{y}}}^{1:P}|{\bf{{x}}}^{1:P}, f_{\text{NeRF}})}_{\text{NeRF model}}
%     \underbrace{p({\bf{{x}}}^{1:P}|{\bf{\widetilde{x}}})}_{\text{Sampling}}.
% \label{eq: rendering}
% \end{equation}
% \begin{equation}
%     p({\bf{\widetilde{y}}}|{\bf{\widetilde{x}}}, f_{NeRF}) \propto
%     \underbrace{p({\bf{\widetilde{y}}}| {\bf{{y}}}^{\mathbf{r}}, {\bf{{x}}}^{\mathbf{r}})}_{\text{Integration}}
%     \underbrace{p({\bf{{y}}}^{\mathbf{r}}|{\bf{{x}}}^{\mathbf{r}}, f_{\text{NeRF}})}_{\text{NeRF model}}
%     \underbrace{p({\bf{{x}}}^{\mathbf{r}}|{\bf{\widetilde{x}}})}_{\text{Sampling}}.
% \label{eq: rendering}
% \end{equation}
% \begin{equation}
%     p({\bf{\widetilde{Y}}}_{T} | {\bf{\widetilde{X}}}_{T}) \varpropto
%     \underbrace{p({\bf{\widetilde{Y}}}_{T} | {\bf{{Y}}}_{T}, {\bf{{X}}}_{T})}_{\text{Integration}}
%     \underbrace{p({\bf{{Y}}}_{T} | {\bf{{X}}}_{T})}_{\text{NeRF Model}}
%     \underbrace{p({\bf{{X}}}_{T} | {\bf{\widetilde{X}}}_{T})}_{\text{Sampling}},
% \label{eq: definiation}
% \end{equation}
\begin{equation}
    p({\bf{\widetilde{Y}}} | {\bf{\widetilde{X}}}) \varpropto
    \underbrace{p({\bf{\widetilde{Y}}} | {\bf{{Y}}}, {\bf{{X}}})}_{\text{Integration}}
    \underbrace{p({\bf{{Y}}} | {\bf{{X}}})}_{\text{NeRF Model}}
    \underbrace{p({\bf{{X}}} | {\bf{\widetilde{X}}})}_{\text{Sampling}}.
\label{eq: probabilitic_NeRF}
\end{equation}
%
% \str{Is $f_\text{NeRF}$ now a random variable? Normally it is not.}
\str{This can also be writtena  more fluently}
The generation process of this probabilistic formulation is as follows.
We first start from (or sample) a set of rays $\widetilde{\mathbf{X}}$.
Conditioning on these rays, we sample 3D points in space $\mathbf{X} \big|\widetilde{\mathbf{X}}$.
Then, we map these 3D points into their colors and density values with the NeRF function, ${\bf{Y}} = f_{\text{NeRF}}({\bf{{X}}})$.
Last, we sample the 2D pixels of the viewing image that corresponds to the 3D ray ${\widetilde{\bf{Y}}}| {\bf{{Y}}}, {\bf{X}}$ with a probabilistic process. This corresponds to integrating colors and densities ${\bf{{Y}}}$ along the ray on locations ${\bf{X}}$.

% In the following sections, we will define the various probabilistic terms.
% \str{Here it would be good to be more explicit and say how are the various probabistic terms are defined. Or we can say that we will specify later, also in the context of Geometric NP. Either way, the current text below looks like deterministic relations, so I think we can not write them down here.}

\str{I suggest we go directly on conditional neural fields. The way we have it now, we only create extra confusion, unless we are the first to propose this decomposition (but there have been other probabilistic NeRFs before, no?). Or perhaps have better structure in the writing, otherwise it is confusing.. What is context, what target?}
The probabilistic model in \cref{eq: probabilitic_NeRF} is for a single 3D object, thus requiring optimizing a function $f_{\text{NeRF}}$ afresh for every new object, which is time-consuming. For NeRF generalization, we accelerate learning and improve generalization by amortizing the probabilistic model over multiple objects, obtaining per-object reconstructions by conditioning on context sets ${{\widetilde {\bf{X}}}_C, {\widetilde {\bf{Y}}}_C}$.
% \str{What about $\widetilde {\bf{X}}_T$? What is that? Also, why (1) has small letters, and here we have capitals?}
% These context variables are few observations from any new object, that is, the rays and the corresponding observed colors.
For clarity, we use ${(\cdot)}_{C}$ to indicate context sets with {a few new observations for a new object}, while ${(\cdot)}_{T}$ indicates target sets containing 3D points or camera rays from novel views of the same object.
Thus, we formulate a probabilistic NeRF for generalization as:
% \str{update this according to the above equation}
%
\begin{equation}
\begin{aligned}
    &p({\bf{\widetilde{Y}}}_{T} | {\bf{\widetilde{X}}}_{T}, {\bf{\widetilde{X}}}_{C}, {\bf{\widetilde{Y}}}_{C}) \varpropto \\
&    \underbrace{p({\bf{\widetilde{Y}}}_{T} | {\bf{{Y}}}_{T}, {\bf{{X}}}_{T})}_{\text{Integration}}
    \underbrace{p({\bf{{Y}}}_{T} | {\bf{{X}}}_{T}, {\bf{\widetilde{X}}}_{C}, {\bf{\widetilde{Y}}}_{C})}_{\text{NeRF Generalization}}
    \underbrace{p({\bf{{X}}}_{T} | {\bf{\widetilde{X}}}_{T})}_{\text{Sampling}}.
\end{aligned}
\label{eq: probabilitic_NeRF_generalization}
\end{equation}
%
%\str{Not sure if this sentence is good enough, please check later again.}
As this paper focuses on generalization with new 3D objects, we keep the same sampling and integrating processes as in ~\cref{eq: probabilitic_NeRF}. We turn our attention to the modeling of the predictive distribution $p({\bf{{Y}}}_{T}| {\bf{{X}}}_{T}, {\bf{\widetilde{X}}}_{C}, {\bf{\widetilde{Y}}}_{C})$ in the generalization step, which implies inferring the NeRF function.

\paragraph{Misalignment between 2D context and 3D structures} It is worth mentioning that the predictive distribution in 3D space is conditioned on 2D context pixels with their ray $\{{\bf{\widetilde{X}}}_{C}, {\bf{\widetilde{Y}}}_{C}\}$ and 3D target points ${\bf{X}}_{T}$, which is challenging due to potential information misalignment. Thus, we need strong inductive biases with 3D structure information to ensure that 2D and 3D conditional information is fused reliably.


% \str{Why do you call this the query step?}

% #############################
% By inferring the function distribution $p(f_{\text{NeRF}})$ from the context sets, we can obtain the predictive distribution as: 
% %
% \begin{equation}
%       p({\bf{Y}}_{T}| {\bf{X}}_{T}, {\bf{\widetilde{X}}}_{C}, {\bf{\widetilde{Y}}}_{C})  
%       = \int p({\bf{Y}}_{T}|f_{\text{NeRF}}, {\bf{X}}_{T}) p(f_{\text{NeRF}}| {{\bf{{X}}}_{T}, \bf{\widetilde{X}}}_{C}, {\bf{\widetilde{Y}}}_{C}) df_{\text{NeRF}} 
% \label{eq: gp_w/o_B}
% \end{equation}
% %
% where $p(f_{\text{NeRF}}| {\bf{X}}_{T} {\bf{\widetilde{X}}}_{C}, {\bf{\widetilde{Y}}}_{C})$ is the prior distribution of the NeRF function, and $p({\bf{Y}}_{T}|f_{\text{NeRF}}, {\bf{X}}_{T})$ is the likelihood term. We integrate the likelihood term over the latent space of all possible NeRF functions.
% %\str{The following two sentences may beed to be rewritten.}
% %It is important to note that the context variables by nature contain fewer views and thus less information per a new object.
% It is worth mentioning that inferring the NeRF function needs to incorporate 2D context pixels with their ray $\{{\bf{\widetilde{X}}}_{C}, {\bf{\widetilde{Y}}}_{C}\}$ and 3D target points ${\bf{X}}_{T}$, which is challenging due to potential information misalignment.  Thus, we need strong inductive biases with 3D structure information to ensure that 2D and 3D conditional information is fused reliably.
% #############################

% \subsection{Geometric Neural Processes for NeRF} 
\subsection{Geometric Bases} 
\label{sec: geometrybases}
% In NeRF generalization, given that the context set is expected to correspond to too few views with few 3D information, 
% % In NeRF generalization, given the context set corresponding to too few 2D views providing few 3D information, 
% fitting a model for $p({\bf{Y}}_{T}| {\bf{X}}_{T}, {\bf{\widetilde{X}}}_{C}, {\bf{\widetilde{Y}}}_{C})$ that generalizes well is challenging. 
To mitigate the information misalignment between 2D context views and 3D target points, we introduce geometric bases ${\bf{{B}}}_{C}=\{{\bf{b}}_i\}_{i=1}^{M}$, which {induces prior structure to the context set} $\{{\bf{\widetilde{X}}}_{C}, {\bf{\widetilde{Y}}}_{C}\}$ geometrically. $M$ is the number of geometric bases. 

\begin{figure*}[t]
  \centering  \includegraphics[width=0.99\textwidth]{ICLR2025/Figures/architecture-0.pdf} % Adjust the size and filename as needed
  % \vspace{-2mm}
\caption{\textbf{Illustration of our Geometric Neural Processes.} 
% We solve the problem of radiance field generalization by Neural Processes. 
% captures uncertainty induced by few available observations.
We cast radiance field generalization as a probabilistic modeling problem. Specifically, we first construct geometric bases ${\bf{B}}_C$ in 3D space from the 2D context sets ${\bf{\widetilde{X}}}_{C}, {\bf{\widetilde{Y}}}_{C}$ to model the 3D NeRF function (Section~\ref{sec: geometrybases}). We then infer the NeRF function by modulating a shared MLP through hierarchical latent variables ${\bf{z}}_{o}, {\bf{z}}_{r}$ and make predictions by the modulated MLP (Section~\ref{sec: hierar}). 
  The posterior distributions of the latent variables are inferred from the target sets ${\bf{\widetilde{X}}}_{T}, {\bf{\widetilde{Y}}}_{T}$, which supervises the priors during training (Section~\ref{sec: object}). 
  } % Caption for the figure
  \label{fig: framework}
  %\vspace{-2mm}
\end{figure*}

\str{where is the semantic representation coming from? Self-supervised models? Or is it learned?}
Each geometric basis consists of a Gaussian distribution in the 3D point space and a semantic representation, \textit{i.e.,} ${\bf{b}}_i = \{ \mathcal{N}(\mu_i, \Sigma_i); \omega_i\}$, 
%\str{What is $\omega_i$ in the equation? The weight of the Gaussian?We have mixtures of Gaussians? Please clarify.} 
where $\mu_i$ and $\Sigma_i$ are the mean and covariance matrix of $i$-th Gaussian in 3D space, and $\omega_i$ is its corresponding latent representation. 
Intuitively, the mixture of all 3D Gaussian distributions implies the structure of the object, while $\omega_i$ stores the corresponding semantic information.
% from a 2D context set, e.g., color and texture. 
In practice, we use a transformer-based encoder to learn the Gaussian distributions and representations from the context sets, \textit{i.e.,} $\{(\mu_i, \Sigma_i, \omega_i)\} = \texttt{Encoder} [{\bf{\widetilde{X}}}_{C}, {\bf{\widetilde{Y}}}_{C}]$. Detailed architecture of the encoder is provided in Appendix~\ref{supp:gaussian}. 

% \begin{equation}
%     {\bf{{B}}}_{C} = \{{\bf{b}}_i\}_{i=1}^{M}, {\bf{b}}_i=\{\mathcal{N}(\mu_i, \Sigma_i); \omega_i\},
%     \\
%      \mu_i, \Sigma_i, \omega_i = \texttt{Encoder} [{\bf{\widetilde{X}}}_{C}, {\bf{\widetilde{Y}}}_{C}],
% \end{equation}
% where $M$ is the number of Gaussian bases. 

% where ${\bf{{B}}}_{C}$ are Gaussian bases inferred from the context views $\{{\bf{\widetilde{X}}}_{C}, {\bf{\widetilde{Y}}}_{C}\}$ with 3D structure information, \textit{i.e.,} 
% ${\bf{{B}}}_{C}=\texttt{Encoder}\Big({\bf{\widetilde{X}}}_{C}, {\bf{\widetilde{Y}}}_{C}\Big)$. 


% To address the information loss in the context views, we develop a geometry-aware prior distribution for the NeRF function. The geometry-aware prior integrates a set of geometry bases ${\bf{{B}}}_{C}$ and the target location points ${\bf{X}}_{T}$, which enrich the context sets with the {structure locality information}. 
% By doing so, we reformulate the prior distribution of the NeRF function as:
% \begin{equation}
%     p(f_{\text{NeRF}}| {\bf{X}}_{T}, {\bf{\widetilde{X}}}_{C}, {\bf{\widetilde{Y}}}_{C}) = p(f_{\text{NeRF}}| {\bf{X}}_{T}, {\bf{{B}}}_{C}), 
% \label{eq: prior_f}
% \end{equation}
% \str{Can a deterministic variable be part of a probabilistic expression?d}
% where ${\bf{{B}}}_{C}$ is a set of Gaussian bases inferred from the context views $\{{\bf{\widetilde{X}}}_{C}, {\bf{\widetilde{Y}}}_{C}\}$ with 3D structure information, \textit{i.e.,} ${\bf{{B}}}_{C}=\texttt{Encoder}[{\bf{\widetilde{X}}}_{C}, {\bf{\widetilde{Y}}}_{C}]$. 
% Specifically, we construct ${\bf{{B}}}_{C}$ as:
% Geometry basis-agnostic ideas, like 4D scene tensor~\cite{chen2022tensorf}, and RBF kernels~\cite{chen2023neurbf} has been used in deterministic NeRF to store the 3D scene geometry and semantic information. This motivates us to use a set of geometry bases to represent both the geometry structure and semantic information of the scene. 
% We assume the space is spanned by a set of basis, with geometric shapes and high-dimensional representation. 
% The geometry basis ${\bf{B}}_C$ is given by a posterior distribution, $p_{\pi}( {\bf{{B}}}_{C}| {\bf{\widetilde{X}}}_{C}, {\bf{\widetilde{Y}}}_{C})$. This can be explained as the posterior knowledge (color and spatial location) of the scene when a human sees a view of a scene (context image). Then, we model the function distribution as:
% \begin{align}
%     &{\bf{{B}}}_{C} = \{{\bf{b}}_i\}_{i=1}^{M}, {\bf{b}}_i=\{\mathcal{N}(\mu_i, \Sigma_i); \omega_i\},
%     \label{eq: generation_B_1}
%     \\
%     & \mu_i, \Sigma_i = \texttt{Att}({\bf{\widetilde{X}}}_{C}, {\bf{\widetilde{Y}}}_{C}), \texttt{Att}({\bf{\widetilde{X}}}_{C}, {\bf{\widetilde{Y}}}_{C}),
%     \label{eq: generation_B_2}
%     \\
%     & \omega_i = \texttt{Att}({\bf{\widetilde{X}}}_{C}, {\bf{\widetilde{Y}}}_{C}),
%     \label{eq: generation_B_3}
% \end{align}
% where $M$ is the number of the Gaussian bases. $\mu \mathbb \in {R}^3$ is the Gaussian center, $\Sigma \in  \mathbb{R}^{3\times 3}$ is the covariance matrix, and $\omega \in \mathbb{R}^{d_B}$ is the corresponding ${d_B}$-dimension semantic representation. 
%Each Gaussian basis represents a 3D Gaussian kernel and its corresponding semantic information. The shape of a Gaussian kernel can reflect a local object structure.
%For each kernel, \js{details here: we use a visual self-attention to estimate the mean $\mu \mathbb \in {R}^3$ and covariance matrix $\Sigma \in  \mathbb{R}^{3\times 3}$, and a corresponding ${d_B}$-dimension semantic representation $\omega \in \mathbb{R}^{d_B}$. }

With the geometric bases $\mathbf{B}_C$, we review the predictive distribution from  $p({\bf{Y}}_{T}| {\bf{X}}_{T}, {\bf{\widetilde{X}}}_{C}, {\bf{\widetilde{Y}}}_{C})$ to $p({\bf{Y}}_{T}| {\bf{X}}_{T},{\bf{{B}}}_{C})$.  By inferring the function distribution $p(f_{\text{NeRF}})$, we reformulate the predictive distribution as: 
\begin{equation}
    % p({\bf{{Y}}}_{T} | {\bf{{X}}}_{T}, {\bf{\widetilde{X}}}_{C}, {\bf{\widetilde{Y}}}_{C}) = 
    p({\bf{{Y}}}_{T} | {\bf{{X}}}_{T}, {\bf{{B}}}_{C}) = \int p({\bf{Y}}_{T}|f_{\text{NeRF}}, {\bf{X}}_{T}) p(f_{\text{NeRF}}| {\bf{X}}_{T}, {\bf{B}}_{C}) df_{\text{NeRF}},
\label{eq: predictive_w_B}
\end{equation}
where $p(f_{\text{NeRF}}| {\bf{X}}_{T}, {\bf{B}}_{C})$ is the prior distribution of the NeRF function, and $p({\bf{Y}}_{T}|f_{\text{NeRF}}, {\bf{X}}_{T})$ is the likelihood term. 
% We integrate the likelihood term with all possible NeRF functions. 
%\str{How do we do this? The space to integrate over must be huge, no?}
%\str{The following sentence is a bit weird, can you check it again.}
% \wy{We integrate the likelihood term over the latent space of all possible variables for modulating NeRF functions by monte carlo sampling, which can be seen as integrating over a function distribution.}
Note that the prior distribution of the NeRF function is conditioned on the target points ${\bf{X}}_{T}$ and the geometric bases ${\bf{B}}_{C}$. 
Thus, the prior distribution is data-dependent on the target inputs, yielding a better generalization on novel target views of new objects. 
Moreover, since ${\bf{B}}_{C}$ is constructed with continuous Gaussian distributions in the 3D space, the geometric bases can enrich the locality and semantic information of each discrete target point, enhancing the capture of high-frequency details~\citep{chen2023neurbf,chen2022tensorf,muller2022instant}.

% Since ${\bf{B}}_{C}$ is constructed in the 3D space, 3D target points ${\bf{X}}_{T})$ is able to effectively interact with ${\bf{B}}_{C}$, alleviating the information misalignment.

%\zx{We need some advantages of B in this paragraph}
%\zx{maybe also refer some splatting/RBF kernel methods to introduce what B is, how does B contain 3D structure information}
% \wy{The inferred posterior about the Gaussian bases shapes is able to reflect the object shape, while the semantic posterior (e.g. color and texture) is embedded in the representation of the bases. Moreover, the Gaussian basis spanned in the space is able to help aggregate the locality information for each queried point, which facilitates learning representing high-frequency details~\cite{chen2023neurbf,chen2022tensorf,muller2022instant}.}

% By integrating the prior distribution in equation~\cref{eq: prior_f} into the predictive distribution in equation~\cref{eq: gp_w/o_B}, we replace  $p({\bf{Y}}_{T}| {\bf{X}}_{T}, {\bf{\widetilde{X}}}_{C}, {\bf{\widetilde{Y}}}_{C})$ with $p({\bf{{Y}}}_{T} | {\bf{{X}}}_{T}, {\bf{{B}}}_{C})$.
% The stochastic processes for NeRF with geometry bases are then derived as:
% % With the encoded geometry base ${\bf{B}}_{C}$, we reformulate the querying step as $p({\bf{{Y}}}_{T} | {\bf{{X}}}_{T}, {\bf{{B}}}_{C})$. By integrating the approximated prior with the bases Eq.~\ref{eq: prior_f} into the generative process in Eq.~\ref{eq: gp_w/o_B}, we derive the stochastic processes for NeRF with Geometry Bases as:
% \str{In 3, $p(f_{Nerf})$ is not conditioned on $X_T$. Is there a difference?}
% \begin{equation}
%     % p({\bf{{Y}}}_{T} | {\bf{{X}}}_{T}, {\bf{\widetilde{X}}}_{C}, {\bf{\widetilde{Y}}}_{C}) = 
%     p({\bf{{Y}}}_{T} | {\bf{{X}}}_{T}, {\bf{{B}}}_{C}) = \int p({\bf{Y}}_{T}|f_{\text{NeRF}}, {\bf{X}}_{T}) p(f_{\text{NeRF}}| {\bf{X}}_{T}, {\bf{B}}_{C}) df_{\text{NeRF}}.
% \label{eq: gp_w_B}
% \end{equation}
%
% Inferred from the context-generated 3D information in ${\bf{{B}}}_{C}$, the NeRF function prior $p(f_{\text{NeRF}}|{\bf{X}}_{T}, {\bf{{B}}}_{C})$ reduces the impact of information loss in context views (\wy{due to sampling and integration}) and becomes more suitable for the \zx{query step} $p({\bf{Y}}_{T}|f_{\text{NeRF}}, {\bf{X}}_{T})$ in 3D space.

\subsection{Geometric Neural Processes with Hierarchical Latent Variables}
\label{sec: hierar}

% To achieve the 
With the geometric bases, we propose Geometric Neural Processes (\textbf{\method{}}) by inferring the NeRF function distribution $p(f_{\text{NeRF}}|{\bf{X}}_{T}, {\bf{{B}}}_{C})$ in a probabilistic way.  
% We can generalize NeRF learning and efficiently adapt the functional distribution to new 3D objects.
Based on the probabilistic NeRF generalization in~\cref{eq: probabilitic_NeRF_generalization}, we introduce hierarchical latent variables to encode various spatial-specific information into $p(f_{\text{NeRF}}|{\bf{X}}_{T}, {\bf{{B}}}_{C})$, improving the generalization ability in different spatial levels.
%\str{Make sure that notation is consistent and not overloaded. Eg, $x^r$ rather than $x^\mathbf{r}$ since it is not that we use the $1:P$ somewhere specific, besides it is not clear that this corresponds to a ray, since the $P$ points could be anywhere.}
Since all rays are independent of each other, we decompose the predictive distribution in \cref{eq: predictive_w_B} as:
\begin{equation}
    p({\bf{Y}}_{T}| {\bf{X}}_{T},  {\bf{B}}_{C})  = \prod_{n=1}^{N} p({\bf{y}}_{T}^{\mathbf{r}, n}| {\bf{x}}_{T}^{{\mathbf{r}}, n},  {\bf{B}}_{C}),
\label{eq: predictive_distribution_ray_specific}
\end{equation}
where the target input ${\bf{X}}_{T}$ consists of $N \times P$ location points $\{{\bf{x}}_{T}^{{\mathbf{r}}, n}\}_{n=1}^{N}$ for $N$ rays.


\begin{figure}[htbp]
\centering
\includegraphics[width=0.9\columnwidth]{ICLR2025/Figures/graphical_model2.pdf} 
\caption{\textbf{Graphical model for the proposed geometric neural processes.}}
\label{fig: graphical_model}
\end{figure}

Further, we develop a hierarchical Bayes framework for \method{} to accommodate the data structure of the target input ${\bf{X}}_{T}$ in \cref{eq: predictive_distribution_ray_specific}.
We introduce an object-specific latent variable $\mathbf{z}_o$ and $N$ individual ray-specific latent variables $\{\mathbf{z}_r^{n}\}_{n=1}^{N}$ to represent the randomness of $f_\text{NeRF}$.
% the probabilistic NeRF function. 


\str{The formatting here looks weird. Is this the right template?}
Within the hierarchical Bayes framework, $\mathbf{z}_o$ encodes the entire object information from all target inputs and the geometric bases $\{\mathbf{X}_T, \mathbf{B}_C\}$ in the global level; while every $\mathbf{z}_r^{n}$ encodes ray-specific information from $\{ \mathbf{x}_T^{\mathbf{r}, n}, \mathbf{B}_C\}$ in the local level, which is also conditioned on the global latent variable $\mathbf{z}_o$. 
The hierarchical architecture allows the model to exploit the structure information from the geometric bases $\mathbf{B}_C$ in different levels, improving the model's expressiveness ability.
By introducing the hierarchical latent variables in \cref{eq: predictive_distribution_ray_specific}, we model \method{} as:
% \begin{equation}
% \small
%         p({\bf{Y}}_{T}| {\bf{X}}_{T}, {\bf{B}}_{C}) = \int \prod_{n=1}^{N} \Big\{ \int p({\bf{y}}_{T}^{\mathbf{r}, n}| {\bf{x}}_{T}^{\mathbf{r}, n}, {\bf{B}}_{C}, {\bf{z}}_r^n,{\bf{z}}_o, ) p({\bf{z}}_{r}^n| {\bf{z}}_o,  {\bf{x}}_{T}^{\mathbf{r}, n}, {\bf{B}}_C) d {\bf{z}}_r^n \Big\} p({\bf{z}}_o |{\bf{X}}_T, {\bf{B}}_C) d {\bf{z}}_o, 
% \label{eq:ganp-model}
% \end{equation}
{\small
\begin{equation}
\begin{aligned}
        p({\bf{Y}}_{T}| {\bf{X}}_{T}, {\bf{B}}_{C}) &= \int \prod_{n=1}^{N} \Big\{ \int p({\bf{y}}_{T}^{\mathbf{r}, n}| {\bf{x}}_{T}^{\mathbf{r}, n}, {\bf{B}}_{C}, {\bf{z}}_r^n,{\bf{z}}_o ) \\
        &p({\bf{z}}_{r}^n| {\bf{z}}_o,  {\bf{x}}_{T}^{\mathbf{r}, n}, {\bf{B}}_C) d {\bf{z}}_r^n \Big\} p({\bf{z}}_o |{\bf{X}}_T, {\bf{B}}_C) d {\bf{z}}_o,
\end{aligned}
\label{eq:ganp-model}
\end{equation}
}where $p({\bf{y}}_{T}^{\mathbf{r}, n}| {\bf{x}}_{T}^{\mathbf{r}, n}, {\bf{B}}_{C}, {\bf{z}}_o, {\bf{z}}_r^i)$ denotes the ray-specific likelihood term. In this term, we use the hierarchical latent variables $\{{\bf{z}}_o, {\bf{z}}_r^i\}$ to modulate a ray-specific NeRF function $f_{\text{NeRF}}$ for prediction, as shown in Fig.~\ref{fig: framework}.
% In general, we first use the object-specific latent variable $\mathbf{z}_o$ to make $f_{NeRF}$ object-specific. Then, the ray-specific latent variable $\mathbf{z}_r$ to enable $f_{\text{NeRF}}$ to capture the local texture information.
Hence, $f_{\text{NeRF}}$ can explore global information of the entire object and local information of each specific ray, leading to better generalization ability on new scenes and new views.
A graphical model of our method is provided in Fig.~\ref{fig: graphical_model}. 

% As mentioned in Eq.~\ref{eq: definiation}, the target inputs can be obtained by randomly sampling ${\bf{x}}_{T}^{1:P}$ from each ray ${\widetilde{\bf{x}}}_{T}$. Thus, target input ${\bf{X}}_{T}$ consists of $N \times P$ location points $\{{\bf{x}}_{T}^{1:P, n}\}_{n=1}^{N}$ given $N$ rays. 
% Since the rendering of each ray is independently \cite{martin2021nerf}, we reformulate the predictive distribution for NeRF in a ray-specific manner:
% \begin{equation}
%     p({\bf{Y}}_{T}| {\bf{X}}_{T},  {\bf{B}}_{C})  = \prod_{n=1}^{N} p({\bf{y}}_{T}^{1:P, n}| {\bf{x}}_{T}^{1:P, n},  {\bf{B}}_{C}).
% \label{eq: predictive_distribution_ray_specific}
% \end{equation}
% Based on the hierarchical data structure of the target inputs, we design a hierarchical latent variable model. In the proposed model, object-specific latent variables ${\bf{g}}$ encode the entire 3D object information; each ${\bf{g}}$ corresponds $N$ individual ray-specific latent variables $\{{\bf{r}}^{n}\}_{n=1}^{N}$.

%\str{Until here. I will check below tomorrow, but maybe you can use the same style like above, more concise and to the point.}
%\str{In general, we have to explain the hierarchical framework better. What is $g$ for instance. }



% that corresponds to the ray's viewpoint $v$. 

% Each viewing image is rendered from a camera pose by marching rays into the 2D image plane and computing colors.

% To optimize a NeRF function for a 3D object, we only have access to several viewing images and their ray information, \textit{e.g., $p({\bf{\widetilde{y}}}|{\bf{\widetilde{x}}}, f_{NeRF})$}.
% \zx{When learning the NeRF function of a 3D object, we only have access to arbitrary 2D views of the 3D object.
% Each viewing image is rendered from a camera pose by marching rays into the 2D image plane and computing colors.
% can render a viewing image of the object from any camera pose by marching rays into the 2D image plane and computing colors. 
% \str{The notation below looks inconsistent with that of the previou svariable, where we have $c_r$, ...}
% In general, each ray corresponds to a pixel in the 2D image from this view. 
% We use ${\bf{\widetilde{x}}} = [\mathbf{r}_o;\mathbf{r}_d] \in \mathbb{R}^{6}$ and ${\bf{\widetilde{y}}} = [r, g, b] \in \mathbb{R}^{3}$ to denote one specific ray and its corresponding pixel color, respectively. 
% Here $\mathbf{r}_o \in \mathbb{R}^3$ and $\mathbf{r}_d \in \mathbb{R}^3$ denote the origin and the direction of the ray, respectively. Each ray color ${\bf{\widetilde{y}}}$ is the RGB value for the corresponding pixel in the 2D image~\cite{arandjelovic2021nerf}.

% To render the ray color of each pixel, as illustrated in Fig.~\ref{fig:problem}, the volume rendering technique~\cite{kajiya1984ray} is used.
% $P$ discrete location points ${\bf{x}}^{1:P} =\{{\bf{x}}^p\}_{p=1}^P$ are first sampled along the ray, and their densities and colors ${\bf{y}}^{1:P} = \{{\bf{y}}^p\}_{p=1}^P$ are queried by the function $f_{\text{NeRF}}$.
% The information from all discrete locations is then integrated via a rendering equation. 
% % An illustration of the rendering process is shown in Fig.~\ref{fig:problem}.
% We factorize the complete rendering process $p({\bf{\widetilde{y}}}|{\bf{\widetilde{x}}})$ as follows:  
% \begin{equation}
%     p({\bf{\widetilde{y}}}|{\bf{\widetilde{x}}}, f_{NeRF}) \propto
%     \underbrace{p({\bf{\widetilde{y}}}| {\bf{{y}}}^{1:P}, {\bf{{x}}}^{1:P})}_{\text{Integration}}
%     \underbrace{p({\bf{{y}}}^{1:P}|{\bf{{x}}}^{1:P}, f_{NeRF})}_{\text{NeRF model}}
%     \underbrace{p({\bf{{x}}}^{1:P}|{\bf{\widetilde{x}}})}_{\text{Sampling}},
% \label{eq: rendering}
% \end{equation}
% \begin{equation}
%     p({\bf{\widetilde{y}}}|{\bf{\widetilde{x}}}) \varpropto p({\bf{\widetilde{y}}}| {\bf{{y}}}_{1:P}, {\bf{{x}}}_{1:P}) p({\bf{{y}}}_{1:P}|{\bf{{x}}}_{1:P})p({\bf{{x}}}_{1:P}|{\bf{\widetilde{x}}}),
% \label{eq: rendering}
% \end{equation}
% where $p({\bf{\widetilde{y}}}| {\bf{{y}}}^{1:P}, {\bf{{x}}}^{1:P})$ represents the integrating step
% % , where the pre-defined render equation computes the ray color 
% by weighted mixing all location colors using the pre-defined render equation ${\bf{\widetilde{y}}} = f_{\text{render}}({\bf{y}}^{1:P}, {\bf{x}}^{1:P})$  \cite{arandjelovic2021nerf,mildenhall2021nerf}.
% % etails of the equation can be found in~\cite{arandjelovic2021nerf,mildenhall2021nerf}.
% $p({\bf{y}}^{1:P}|{\bf{x}}^{1:P})$ denotes the NeRF modeling step for each queried points, \textit{e.g.}, ${\bf{y}}^{1:P}:= f_{\text{NeRF}}({\bf{x}}^{1}), f_{\text{NeRF}}({\bf{x}}^{2}), ..., f_{\text{NeRF}}({\bf{x}}^{P})$.
% $p({\bf{{x}}}^{1:P}|{\bf{\widetilde{x}}})$ denotes the randomly sampling step along the ray $\bf{\widetilde{x}}$. 
% \zx{Given a set of rays ${\bf{\widetilde{X}}}=\{ {\bf{\widetilde{x}}} \}^{N}$ from the same camera pose, we can obtain its corresponding 2D image ${\bf{\widetilde{Y}}}= \{ {\bf{\widetilde{y}}} \}^{N}$ consisting of all pixel colors by ray-specific rendering. Each specific ray corresponds to a pixel on the image.}
% Moreover, we use ${\bf{\widetilde{X}}}$ and ${\bf{\widetilde{Y}}}$ to represent sets of rays and their corresponding colors in 2D image plane.


% \subsection{Probabilistic Radiance Field Generalization} 

% Conventional methods~\cite{martin2021nerf,chen2022tensorf} usually train a deterministic neural network to optimize the NeRF function $f_{\text{NeRF}}$ in Eq. \ref{eq: rendering}. However, this requires the model to overfit large amounts of viewing images for each 3D object, which is data intensive and time-consuming, with poor generalization ability.

%However, it is difficult to collect location points and their location densities and colors in 3D space (\textcolor{red}{citation}). 
% By contrast, this paper focuses on radiance field generalization on arbitrary new 3D objects with few viewing images. 
% However, the method is applicable to arbitrary implicit neural representation (e.g. 2D images). 
% For a new 3D object
% Therefore, $f_{\text{NeRF}}$ needs to be quickly generalized to a new scene based on \textit{few-shot} context views $\{ {\bf{\widetilde{X}}}_C, {\bf{\widetilde{Y}}}_C\}$. 
% %images and their ray information, which are represented as the context set including ray and pixel color $\{ {\bf{\widetilde{X}}}_C, {\bf{\widetilde{Y}}}_C\}$. 
% The generalized NeRF function is then utilized to render any target set of ray ${\bf{\widetilde{X}}}_{T}$ to get the corresponding pixel color set ${\bf{\widetilde{Y}}}_{T}$ in 2D image plane.

% To achieve fast generalization with limited views, we formulate the problem of radiance field generalization in a probabilistic manner.
% The probabilistic formulation enables us to infer the NeRF function while considering uncertainty, improving the generalization ability on limited context data.
% Formally, we formulate the goal of radiance field generalization as $p({\bf{\widetilde{Y}}}_{T}| {\bf{\widetilde{X}}}_{T}, {\bf{\widetilde{X}}}_{C}, {\bf{\widetilde{Y}}}_{C} )$. 
% % The target distribution of radiance field generalization is $p({\bf{\widetilde{Y}}}_{T}| {\bf{\widetilde{X}}}_{T}, {\bf{\widetilde{X}}}_{C}, {\bf{\widetilde{Y}}}_{C} )$. 
% Considering the rendering with a NeRF function in Eq.~\ref{eq: rendering}, we review the target distribution as:
% % \begin{equation}
% %     p({\bf{\widetilde{Y}}}_{T} | {\bf{\widetilde{X}}}_{T}, {\bf{\widetilde{X}}}_{C}, {\bf{\widetilde{Y}}}_{C}) \varpropto
% %     \underbrace{p({\bf{\widetilde{Y}}}_{T} | {\bf{{Y}}}_{T}, {\bf{{X}}}_{T})}_{\text{Integration}}
% %     \underbrace{p({\bf{{Y}}}_{T} | {\bf{{X}}}_{T}, {\bf{\widetilde{X}}}_{C}, {\bf{\widetilde{Y}}}_{C})}_{\text{Generalization}}
% %     \underbrace{p({\bf{{X}}}_{T} | {\bf{\widetilde{X}}}_{T})}_{\text{Sampling}},
% % \label{eq: definiation}
% % \end{equation}
% \begin{equation}
%     p({\bf{\widetilde{Y}}}_{T} | {\bf{\widetilde{X}}}_{T}, {\bf{\widetilde{X}}}_{C}, {\bf{\widetilde{Y}}}_{C}) \varpropto
%     \underbrace{p({\bf{\widetilde{Y}}}_{T} | {\bf{{Y}}}_{T}, {\bf{{X}}}_{T})}_{\text{Integration}}
%     \underbrace{p({\bf{{Y}}}_{T} | {\bf{{X}}}_{T}, {\bf{\widetilde{X}}}_{C}, {\bf{\widetilde{Y}}}_{C})}_{\text{Generalization}}
%     \underbrace{p({\bf{{X}}}_{T} | {\bf{\widetilde{X}}}_{T})}_{\text{Sampling}},
% \label{eq: definiation}
% \end{equation}
% Without loss of generality, we share the fixed sampling and integrating processes as in Eq.~\ref{eq: rendering}. Thus, we focus on the modeling of query step $p({\bf{{Y}}}_{T}| {\bf{{X}}}_{T}, {\bf{\widetilde{X}}}_{C}, {\bf{\widetilde{Y}}}_{C})$.  

%\wy{The ray casting used in volume rendering (sampling process described above) enables sampling in the 3D space continuously, which }
% The probabilistic formulation enables us to obtain the NeRF function by neural processes, which capture uncertainty and directly infer the function in a single feed-forward pass. 
% This leads to both effective and efficient generalization of the NeRF function on new scenes.


% Conventional methods \zx{references\cite{}} usually learn a deterministic neural network $\theta_{NeRF}$ to model a NeRF function. This requires the neural network $\theta_{NeRF}$ to overfit on amounts of viewing images for a 3D object, which is time-consuming. 
% \begin{equation}
% p({\bf{{Y}}}_{T} | {\bf{{X}}}_{T}, {\bf{\widetilde{X}}}_{C}, {\bf{\widetilde{Y}}}_{C}) \approx  p({\bf{{Y}}}_{T} | {\bf{{X}}}_{T}, \theta^*_{NeRF}), 
% \end{equation}
% where the best neural network is estimated by maximum a posterior (MAP) on the support sets of ray and ray colors, \textit{e.g.}, $\theta^*_{NeRF} =\mathop{\arg\min}_{\theta} p(\theta_{NeRF}|{\bf{\widetilde{X}}}_{C}, {\bf{\widetilde{Y}}}_{C})$. For each new 3D object, $\theta_{NeRF}$ will be re-trained for overfitting, yielding worse generalizations. Hence, leveraging limited viewing images for radiance field generalization remains a problem. 

% \textbf{Neural Processes for Radiance Field Generalization.}
% \js{Motivation of generative processes in a probabilistic way}
% In radiance field generalization, each new 3D object only accesses a few viewing images. In this case, a deterministic NeRF function could not capture uncertainty caused by the limited viewing images, leading to worse generalization ability on new 3D objects. 


% \subsection{Stochastic Processes for Radiance Field Generalization with Geometry Basis} 
% \label{sec: geometrybases}

% \noindent \textbf{Stochastic Processes for NeRF.}
% To capture uncertainty and improve generalization ability on limited context views, we cast radiance field generalization as stochastic processes over the NeRF function in 3D space. 
% {The processes directly infer the NeRF function in a feedforward pass, leading to both effective and efficient generalization on new scenes.}
% Specifically, we formulate the predictive distribution of radiance field generalization as follows:
% \begin{equation}
%       p({\bf{Y}}_{T}| {\bf{X}}_{T}, {\bf{\widetilde{X}}}_{C}, {\bf{\widetilde{Y}}}_{C})  
%       = \int p({\bf{Y}}_{T}|f_{NeRF}, {\bf{X}}_{T}) p(f_{NeRF}| {\bf{\widetilde{X}}}_{C}, {\bf{\widetilde{Y}}}_{C}) df_{NeRF} 
% \label{eq: gp_w/o_B}
% \end{equation}
% where $p(f_{\text{NeRF}}| {\bf{\widetilde{X}}}_{C}, {\bf{\widetilde{Y}}}_{C})$ is a prior distribution of the NeRF function.
% Since $f_{\text{NeRF}}$ is constructed on 3D space, it should ideally be inferred from the 3D location context sets $\{{\bf{{X}}}_{C}, {\bf{{Y}}}_{C}\}$. 
% \str{I am not sure the following sentences really make a (important) point.}
% However, the 3D location information is not available during practice training.
% The only accessible information of the 3D object is the limited viewing images $\{{\bf{\widetilde{X}}}_{C}, {\bf{\widetilde{Y}}}_{C}\}$.
% Moreover, the discrete sampling and integration for rendering results in information loss of the context sets from 3D location space to 2D views (Fig. \ref{fig:problem}).
% Therefore, inferring $f_{\text{NeRF}}$ by the context views is less optimal.
% However, NeRF mapping location points to their location colors and densities should be ideally inferred from the location sets $\{{\bf{{X}}}_{C}, {\bf{{Y}}}_{C}\}$, rather than the ray sets $\{{\bf{\widetilde{X}}}_{C}, {\bf{\widetilde{Y}}}_{C}\}$.
% In practice, the former is not available during training. 
% We can not directly transfer the context sets in the ray or camera space $\{{\bf{{X}}}_{C}, {\bf{{Y}}}_{C}\}$ to the 3D location space $\{{\bf{\widetilde{X}}}_{C}, {\bf{\widetilde{Y}}}_{C}\}$. This is intractable since the information loss of the context sets from the location space (3D) to the ray space (2D) due to the discrete sampling and integration. 

% To better capture the uncertainty with the context views, we cast radiance field generation as a stochastic process over a NeRF function in the 3D space. 
% The prior distribution of the function should be formulated as $p(f_{\text{NeRF}}| {\bf{X}}_{T}, {\bf{{X}}}_{C}, {\bf{{Y}}}_{C})$. 
% However, in practice, ${\bf{{X}}}_{C}, {\bf{{Y}}}_{C}$ (the context radiance field) is not available during training. We can not directly transfer the context sets in the ray or camera space $\{{\bf{{X}}}_{C}, {\bf{{Y}}}_{C}\}$ to the 3D location space $\{{\bf{\widetilde{X}}}_{C}, {\bf{\widetilde{Y}}}_{C}\}$. This is intractable since the information loss of the context sets from the location space (3D) to the ray space (2D) due to the discrete sampling and integration. We introduce a set of geometry basis to address this issue, which can also enrich the query points with the structure locality information.

% Thus, we can factorize the query process in Eq.~\ref{eq: definiation} as:
% \begin{equation}
%     p({\bf{Y}}_{T}| {\bf{X}}_{T}, {\bf{\widetilde{X}}}_{C}, {\bf{\widetilde{Y}}}_{C}) \varpropto p({\bf{Y}}_{T}, f_{NeRF}| {\bf{X}}_{T}, {\bf{{X}}}_{C}, {\bf{{Y}}}_{C}) p( {\bf{{X}}}_{C}, {\bf{{Y}}}_{C} | {\bf{\widetilde{X}}}_{C}, {\bf{\widetilde{Y}}}_{C}),
% \label{eq: query process1}
% \end{equation}
% where $p({\bf{{X}}}_{C}, {\bf{{Y}}}_{C} | {\bf{\widetilde{X}}}_{C}, {\bf{\widetilde{Y}}}_{C})$ denotes generating process from ray to location spaces, which is reverse from the complete rendering from location to ray spaces in Eq.~\ref{eq: rendering}. Therefore, this generating process is intractable since the information loss of the support sets from the location space (3D) to the ray space (2D). 

% \noindent \textbf{Geometry Basis.}
% To address the information loss in the context views, we develop a geometry-aware prior distribution for the NeRF function. The geometry-aware prior integrates a set of geometry bases ${\bf{{B}}}_{C}$ and the target location points ${\bf{X}}_{T}$, which enrich the context sets with the {structure locality information}. 
% By doing so, we reformulate the prior distribution of the NeRF function as:
% \begin{equation}
%     p(f_{\text{NeRF}}| {\bf{X}}_{T}, {\bf{\widetilde{X}}}_{C}, {\bf{\widetilde{Y}}}_{C}) = p(f_{\text{NeRF}}| {\bf{X}}_{T}, {\bf{{B}}}_{C}), 
% \label{eq: prior_f}
% \end{equation}
% \str{Can a deterministic variable be part of a probabilistic expression?d}
% where ${\bf{{B}}}_{C}$ is a set of Gaussian bases inferred from the context views $\{{\bf{\widetilde{X}}}_{C}, {\bf{\widetilde{Y}}}_{C}\}$ with 3D structure information, \textit{i.e.,} ${\bf{{B}}}_{C}=\texttt{Encoder}[{\bf{\widetilde{X}}}_{C}, {\bf{\widetilde{Y}}}_{C}]$. Specifically, we construct ${\bf{{B}}}_{C}$ as:
% % Geometry basis-agnostic ideas, like 4D scene tensor~\cite{chen2022tensorf}, and RBF kernels~\cite{chen2023neurbf} has been used in deterministic NeRF to store the 3D scene geometry and semantic information. This motivates us to use a set of geometry bases to represent both the geometry structure and semantic information of the scene. 
% % We assume the space is spanned by a set of basis, with geometric shapes and high-dimensional representation. 
% % The geometry basis ${\bf{B}}_C$ is given by a posterior distribution, $p_{\pi}( {\bf{{B}}}_{C}| {\bf{\widetilde{X}}}_{C}, {\bf{\widetilde{Y}}}_{C})$. This can be explained as the posterior knowledge (color and spatial location) of the scene when a human sees a view of a scene (context image). Then, we model the function distribution as:
% \begin{align}
%     &{\bf{{B}}}_{C} = \{{\bf{b}}_i\}_{i=1}^{M}, {\bf{b}}_i=\{\mathcal{N}(\mu_i, \Sigma_i); \omega_i\},
%     \label{eq: generation_B_1}
%     \\
%     & \mu_i, \Sigma_i = \texttt{Att}({\bf{\widetilde{X}}}_{C}, {\bf{\widetilde{Y}}}_{C}), \texttt{Att}({\bf{\widetilde{X}}}_{C}, {\bf{\widetilde{Y}}}_{C}),
%     \label{eq: generation_B_2}
%     \\
%     & \omega_i = \texttt{Att}({\bf{\widetilde{X}}}_{C}, {\bf{\widetilde{Y}}}_{C}),
%     \label{eq: generation_B_3}
% \end{align}
% where $M$ is the number of the Gaussian bases. $\mu \mathbb \in {R}^3$ is the Gaussian center, $\Sigma \in  \mathbb{R}^{3\times 3}$ is the covariance matrix, and $\omega \in \mathbb{R}^{d_B}$ is the corresponding ${d_B}$-dimension semantic representation. 
% %Each Gaussian basis represents a 3D Gaussian kernel and its corresponding semantic information. The shape of a Gaussian kernel can reflect a local object structure.
% %For each kernel, \js{details here: we use a visual self-attention to estimate the mean $\mu \mathbb \in {R}^3$ and covariance matrix $\Sigma \in  \mathbb{R}^{3\times 3}$, and a corresponding ${d_B}$-dimension semantic representation $\omega \in \mathbb{R}^{d_B}$. }
% Since the Gaussian bases are continuous in the location space, we can refine arbitrary location points with the Gaussian bases.
% \zx{We need some advantages of B in this paragraph}
% \zx{maybe also refer some splatting/RBF kernel methods to introduce what B is, how does B contain 3D structure information}

% \js{too details, use some \texttt{Atten} to obtain each parameters.}
% Given the context set $[\widetilde{X};\widetilde{Y}] \in \mathbb{R}^{H\times W \times (3+3+3)}$, a visual self-attention module first produces a $M\times D$ tokens with $M$ is the number of visual tokens and $D$ is the hidden dimension. The number of Gaussians we use equals to the number of tokens $M$. Then, we use one MLP to predict centers $\mu$, as well as the rotation $R$ and scaling $S$ matrices parameters for producing covariance matrix $\Sigma$, and one MLP to produce the latent representations $\omega$. The covariance matrix is obtained by $\Sigma^C = RSS^TR^T$.
% \begin{equation}
%     \Sigma = RSS^TR^T.
%     \label{eq:cov-matrix}
% \end{equation}
%where $R\in \mathbb{R}^{3\times3}$ is the rotation matrix, and $S \in \mathbb{R}^3$ is the scaling matrix. 



% The generative process of the NeRF function can be formulated in a probabilistic way:

% Different from previous works, we cast radiance field generalization as a 

% we the distribution over a
% single function $p( )$




% \begin{equation}
%     p({\bf{Y}}_{T}| {\bf{X}}_{T}, {\bf{\widetilde{X}}}_{C}, {\bf{\widetilde{Y}}}_{C}) =  \int p({\bf{Y}}_{T}| f_{NeRF}, {\bf{X}}_{T}) p(f_{NeRF} | {\bf{\widetilde{X}}}_{C}, {\bf{\widetilde{Y}}}_{C}) d f_{NeRF}
% \end{equation}


%To improve the generalization ability and achieve efficient inference on new scenes of Neural Field methods, we propose to learn to infer specific model parameters for each scene by Neural Processes.
%\zx{Advantages}
%In the following, we use NeRF generalization to illustrate the proposed method.  In NeRF generalization, a few views (one or two) of images $I_c$ and its corresponding camera pose $\mathbf{p}$ serve as the context information. 

%We represent each location in this scene by aggregating this Gaussian basis based on the radial basis function (RBF). 
%Then, based on the context information, the task is to estimate an implicit function that can be used to infer the target for unseen views.

% The proposed GP-INR framework assumes a space composed of a set of Gaussian basis that encode the spatial location and semantic information of a scene. Initially, GP-INR predicts a Gaussian basis $B_C$ from the observed context. Similar to the recent advances in implicit neural fields (e.g., Neurbf~\cite{chen2023neurbf}), at arbitrary new locations $X_T \in \mathbb{R}^{N\times P\times 3}$, we aggregate the Gaussians to form a new representation of this location $X'_C$ via the radial basis function (RBF). By averaging the representations both globally and locally along rays, we obtain a global latent $g_C$ and a ray-specific latent $r_C$ to modulate an MLP for predicting the implicit neural field. During training, with the target view and image $I_T$ also provided, we perform the same procedures for $I_T$ and align latent variables from both the context and target. For simplicity, in the following, we will use $I_C$ as an example to illustrate. 

% Introducing B
% ; 2). enrich the query points representation by aggregating the locality scene information

% \noindent \textbf{Stochastic Processes with Geometry Bases.} 
% By integrating the prior distribution with geometry bases ${\bf{B}}_{C}$ (Eq. \ref{eq: prior_f}) into the predictive distribution in Eq. \ref{eq: gp_w/o_B}, we reformulate the predictive distribution $p({\bf{Y}}_{T}| {\bf{X}}_{T}, {\bf{\widetilde{X}}}_{C}, {\bf{\widetilde{Y}}}_{C})$ as $p({\bf{{Y}}}_{T} | {\bf{{X}}}_{T}, {\bf{{B}}}_{C})$.
% The stochastic processes for NeRF with geometry bases are then derived as:
% % With the encoded geometry base ${\bf{B}}_{C}$, we reformulate the querying step as $p({\bf{{Y}}}_{T} | {\bf{{X}}}_{T}, {\bf{{B}}}_{C})$. By integrating the approximated prior with the bases Eq.~\ref{eq: prior_f} into the generative process in Eq.~\ref{eq: gp_w/o_B}, we derive the stochastic processes for NeRF with Geometry Bases as:
% \begin{equation}
%     % p({\bf{{Y}}}_{T} | {\bf{{X}}}_{T}, {\bf{\widetilde{X}}}_{C}, {\bf{\widetilde{Y}}}_{C}) = 
%     p({\bf{{Y}}}_{T} | {\bf{{X}}}_{T}, {\bf{{B}}}_{C}) = \int p({\bf{Y}}_{T}|f_{NeRF}, {\bf{X}}_{T}) p(f_{NeRF}| {\bf{X}}_{T}, {\bf{B}}_{C}) df_{NeRF}.
% \label{eq: gp_w_B}
% \end{equation}
% Inferred from the context-generated 3D information in ${\bf{{B}}}_{C}$, the NeRF function prior $p(f_{\text{NeRF}}|{\bf{X}}_{T}, {\bf{{B}}}_{C})$ reduces the impact of information loss in context views and becomes more suitable for the \zx{query step} $p({\bf{Y}}_{T}|f_{\text{NeRF}}, {\bf{X}}_{T})$ in 3D space.
% Moreover, since we consider the target location information ${\bf{X}}_{T}$ as well in $p(f_{\text{NeRF}}|{\bf{X}}_{T}, {\bf{{B}}}_{C})$, the NeRF function $f_{\text{NeRF}}$ is more generalizable to new views of new objects.

% This formulation provides a proxy between 2D context information and the 3D space by representing the 3D space with the continuous Gaussian basis. $p(f_{\text{NeRF}}|{\bf{X}}_{T}, {\bf{{B}}}_{C})$ is the conditional function distribution where we sample the modulation variable to modulate a shared MLP as the NeRF function, and $p({\bf{Y}}_{T}|f_{\text{NeRF}}, {\bf{X}}_{T})$ is NeRF \zx{rendering process}. We provide a new perspective to model the function distribution fully in 3D space. By doing so, we eliminate the information loss from 2D context to 3D location space.

% \begin{equation}
%     X'_T = \text{MLP}(\sum_i^{M} \varphi(x, \mu_i, \Sigma_i)\omega_i)
% \end{equation}s

% \begin{equation}
%     \varphi(x, \mu_i, \Sigma_i) = \exp (-(x-\mu_i)^T\Sigma_i^{-1}(x-\mu_i) /2)
% \end{equation}

%Hence, instead of directly using the 2D context set, we update the Gaussian basis (both shape and representation) in 3D space. Then, it is natural to use a continuous aggregation function (e.g. Gaussian radial basis function) to enrich the information at each location. By doing so, we eliminate the information loss from 2D context to 3D location space. 




% \subsection{Modeling of Geometry-aware Neural Processes}
% \subsection{Geometry-aware Neural Processes with Hierarchical Modulation}
% \label{sec: hierar}

% % To achieve the 
% To implement the inference of the NeRF function, we propose the Geometric Neural Process (\textbf{GeomNP}) for radiance field generalization, which efficiently adapt the functional distribution to new 3D objects. Specifically, \textbf{GeomNP} are constructed on a hierarchical Bayes framework. For 3D objects, the framework encodes object-specific and ray-specific latent variables in different levels, which helps the developed model querying the structure information from the Geometry bases $\mathbf{B}_C$. 

% \zx{why and how neural processes?}
% In this section, we present how to perform the \zx{rendering process} $p({\bf{Y}}_{T}| {\bf{X}}_{T},  {\bf{B}}_{C})$, including sampling a function from $p(f_{\text{NeRF}}|{\bf{X}}_{T}, {\bf{{B}}}_{C})$. 

% \noindent{{\textbf{Hierarchical Latent Variables.}}}
% The motivation of hierarchical latent variables in our model is the data structure of target inputs ${\bf{X}}_{T}$.
% As mentioned in Eq.~\ref{eq: definiation}, the target inputs can be obtained by randomly sampling ${\bf{x}}_{T}^{1:P}$ from each ray ${\widetilde{\bf{x}}}_{T}$. Thus, target input ${\bf{X}}_{T}$ consists of $N \times P$ location points $\{{\bf{x}}_{T}^{1:P, n}\}_{n=1}^{N}$ given $N$ rays. 
% Since the rendering of each ray is independently \cite{martin2021nerf}, we reformulate the predictive distribution for NeRF in a ray-specific manner:
% \begin{equation}
%     p({\bf{Y}}_{T}| {\bf{X}}_{T},  {\bf{B}}_{C})  = \prod_{n=1}^{N} p({\bf{y}}_{T}^{1:P, n}| {\bf{x}}_{T}^{1:P, n},  {\bf{B}}_{C}).
% \label{eq: predictive_distribution_ray_specific}
% \end{equation}
% Based on the hierarchical data structure of the target inputs, we design a hierarchical latent variable model. In the proposed model, object-specific latent variables ${\bf{g}}$ encode the entire 3D object information; each ${\bf{g}}$ corresponds $N$ individual ray-specific latent variables $\{{\bf{r}}^{n}\}_{n=1}^{N}$.

% \begin{wrapfigure}{r}{0.5\textwidth}
% \vspace{-5mm}
% \centering
% \centerline{
% \includegraphics[width=0.45\columnwidth]{Figures/graphical_model.png} 
% } 
% \vspace{-2mm}
% \caption{\textbf{Graphical model for the proposed geometric neural processes.}
% }
% \vspace{-2mm}
% \label{fig: graphical_model}
% \end{wrapfigure}
%${\mathbf{z}_o}$

% \subsection{Inferring with Geometric Bases and Modulation}

% \str{The following paragraph is not very clear.}

In the modeling of {\method{}}, the prior distribution of each hierarchical latent variable is conditioned on the geometric bases and target input. 
%\textcolor{blue}{To infer each latent variable, we first integrate the geometric bases and each target input, yielding a location representation specific to the target input. The location representation has access to relevant locality information from the geometry bases, \textit{i.e.}, $<{\bf{x}}_{T}^{\mathbf{r}, n}, {\bf{B}}_C >$. }
% For generalization, we need to infer latent variables that are specific to the target input. 
% To this end, 
We first represent each target location by integrating the geometric bases, \textit{i.e.}, $<{\bf{x}}_{T}^{n}, {\bf{B}}_C >$, which aggregates the relevant locality and semantic information for the given input. 
Since ${\bf{B}}_{C}$ contains $M$ Gaussians, we employ a Gaussian radial basis function in \cref{eq:rbf_agg} between each target input ${\bf{x}}_{T}^{ n}$ and each geometric basis ${\bf{b}}_i$ to aggregate the structural and semantic information to the 3D location representation. Thus, we obtain the 3D location representation as follows:
\begin{equation}
\label{eq:rbf_agg}
    <{\bf{x}}_{T}^{n}, {\bf{B}}_C > = \texttt{MLP}\Big[\sum_i^{M} \exp (-\frac{1}{2}({\bf{x}}_{T}^{n}-\mu_i)^T\Sigma_i^{-1}({\bf{x}}_{T}^{n}-\mu_i) ) \cdot \omega_i\Big],
\end{equation} 
where $\texttt{MLP}[\cdot]$ is a learnable neural network.
With the location representation $<{\bf{x}}_{T}^{n}, {\bf{B}}_C >$, we next infer each latent variable hierarchically, in object and ray levels. 

\noindent {\textbf{Object-specific Latent Variable.}} The distribution of the object-specific latent variable ${\bf{z}}_o$ is obtained by aggregating all location representations:
\begin{equation}
    [\mu_{{o}}, \sigma_{{o}}] 
    = \texttt{MLP}\Big[\frac{1}{N \times P}\sum_{n = 1}^{N}\sum_{\mathbf{r}}
    <{\bf{x}}_{T}^{n}, {\bf{B}}_C >\Big],
\end{equation} 
where we assume $p({\bf{z}}_o | {\bf{B}}_C,  {\bf{X}}_T)$ is a standard Gaussian distribution and generate its mean $\mu_{o}$ and variance $\sigma_{o}$ by a ~\texttt{MLP}. 
Thus, our model captures objective-specific uncertainty in the NeRF function.


\noindent {\textbf{Ray-specific Latent Variable.}} 
% By ray-specific latent variable, the object-specific is expected to capture the local details.
To generate the distribution of the ray-specific latent variable, we first average the location representations ray-wisely. 
We then obtain the ray-specific latent variable by aggregating the averaged location representation and the object latent variable through a lightweight transformer. We formulate the inference of the ray-specific latent variable as:
\begin{equation}
    [\mu_{{r}}, \sigma_{{r}}] = \texttt{Transformer} \Big[\texttt{MLP}[\frac{1}{P}\sum_{\mathbf{r}}
    <{\bf{x}}_{T}^{n}, {\bf{B}}_C >]; \hat{{\bf{z}}}_o \Big],
\end{equation}
where $\hat{{\bf{z}}}_o$ is a sample from the prior distribution $p({\bf{z}}_o | {\bf{X}}_T, {\bf{B}}_C)$. 
Similar to the object-specific latent variable, we also assume the distribution $p({\bf{z}}_r^n| {\bf{z}}_o,  {\bf{x}}_{T}^{\mathbf{r}, n}, {\bf{B}}_C)$ is a mean-field Gaussian distribution with the mean $\mu_{{r}}$ and variance $\sigma_{{r}}$. We provide more details of the latent variables in Appendix~\ref{supp:latent-variables}.

% The detail of the used Transformer is given in the Appendix. In summary, our latent variable is in a hierarchical structure. 
% The location-specific latent variable $r_C$ is to modulate the NeRF function specific to the queried ray (or pixel location in 2D image). We infer a ray-specific variable $r_c$ by first aggregating the feature ray-wisely:
% \begin{equation}
%     r'_c = \text{MLP}(\frac{1}{ P}\sum_j^{P}(\bf{X}'_T)[j])
% \end{equation}


%Then, we perform a hierarchical formulation by incorporating the global variable to obtain the ray-specific variable. This enables us to design the latent variable in a hierarchical structure, which is rational as it learns the scene coarse-to-fine. 

% Then, $r_c$ is obtained by feeding $r'_c$ together with the sampled $\hat{g}_c$ into a Transformer: 
% \begin{equation}
%     r_c = [\mu^c_r, \sigma^c_r] = \text{Transformer}([\hat{g}_c; \hat{r}_C]),
% \end{equation}
% where $\mu^r_g$ and $\sigma^r_g$ are the mean and variance of global variables, respectively. The detail of the used Transformer is given in the Appendix. In summary, our latent variable is in a hierarchical structure. 

\noindent  \textbf{NeRF Function Modulation.}
With the hierarchical latent variables $\{{\bf{z}}_o, {\bf{z}}_r^n\}$, we modulate a neural network for a 3D object in both object-specific and ray-specific levels.  Specifically, the modulation of each layer is achieved by scaling its weight matrix with a style vector~\citep{guo2023versatile}. 
The object-specific latent variable ${\bf{z}}_o$ and ray-specific latent variable ${\bf{z}}_r^n$ are taken as style vectors of the low-level layers and high-level layers, respectively. The prediction distribution $p({\bf{Y}}_{T}| {\bf{X}}_{T}, {\bf{B}}_{C})$ are finally obtained by passing each location representation through the modulated neural network for the NeRF function. 
More details are provided in Appendix~\ref{supp:modulate}. 
% The modulated MLP layer used in our paper is similar to the style \textit{modulation} in ~\cite{guo2023versatile}. Essentially, we predict a style vector $s\in \mathbb{R}^{d_{in}}$ to multiply or scale the weight matrix of an MLP, $W \in \mathbb{R}^{d_{in} \times d_{out}}$.


% \subsection{Inference of Geometry-aware Neural Processes}
% \label{sec: elbo}
% ELBO

% \noindent{\textbf{Variational Posteriors with the Geometry Bases.}} Solving \textbf{GANPs} with Eq.~\ref{eq:ganp-model} involves estimating the true posterior, $p({\bf{g}},  \{{\bf{r}}_i\}_{r=1}^{N_{ray}} | {\widetilde{\bf{X}}}_T, {\widetilde{\bf{Y}}}_T)$ which is intractable. Hence, we introduce a variational posterior distribution, which can be factorized as follows:
% \begin{equation}
% p({\bf{g}},  \{{\bf{r}}_i\}_{r=1}^{N_{ray}} | {\widetilde{\bf{X}}}_T, {\widetilde{\bf{Y}}}_T) \approx q_{\theta, \phi}({\bf{g}},  \{{\bf{r}}_i\}_{r=1}^{N_{ray}} | {\bf{X}}_T, {\bf{B}}_T),
% \end{equation}

\subsection{Empirical Objective}
\label{sec: object}

\noindent{\textbf{Evidence Lower Bound.}} 
To optimize the proposed \method{},
we apply variational inference~\citep{garnelo2018neural} and derive the evidence lower bound (ELBO) as:
\begin{equation}
\begin{aligned}
% \mathcal{L}_{\text{ELBO}}
& \log   p({\bf{Y}}_{T}| {\bf{X}}_{T}, {\bf{B}}_{C})
\geq \\
&\mathbb{E}_{q({\bf{z}}_o | {\bf{B}}_T,  {\bf{X}}_T)}  \Big\{  \sum_{n=1}^{N}  \mathbb{E}_{q({\bf{z}}_r^n| {\bf{z}}_o,  {\bf{x}}_{T}^{\mathbf{r}, n}, {\bf{B}_T})} \log p({\bf{y}}_{T}^{{\mathbf{r}}, n}| {\bf{x}}_{T}^{{\mathbf{r}}, n}, {\bf{z}}_o, {\bf{z}}_r^n) \\
&- D_{\text{KL}}[q({\bf{z}}_r^n| {\bf{z}}_o,  {\bf{x}}_{T}^{{\mathbf{r}}, n}, {{\bf{B}}_T}) || p({\bf{z}}_r^n| {\bf{z}}_o,  {\bf{x}}_{T}^{{\mathbf{r}}, n}, {{\bf{B}}_C}) ] \Big\} \\
& - D_{\text{KL}}[q({\bf{z}}_o | {\bf{B}}_T,  {\bf{X}}_T) || p({\bf{z}}_o | {\bf{B}}_C,  {\bf{X}}_T)], \\
\end{aligned}
\end{equation}
where $q_{\theta, \phi}({\bf{z}}_o,  \{{\bf{z}}_r^i\}_{i=1}^{N} | {\bf{X}}_T, {\bf{B}}_T) = \Pi_{i=1}^{N}q({\bf{z}}_r^n| {\bf{z}}_o,  {\bf{x}}_{T}^{{\mathbf{r}}, n}, {{\bf{B}}_T}) q({\bf{z}}_o | {\bf{B}}_T,  {\bf{X}}_T)$ is the involved variational posterior for the hierarchical latent variables.  ${\bf{B}}_T$ is the geometric bases constructed from the target sets $\{{\bf{\widetilde{X}}}_{T}, {\bf{\widetilde{Y}}}_{T}\}$, which are only accessible during training. 
The variational posteriors are inferred from the target sets during training, which introduces more information on the object. 
The prior distributions are supervised by the variational posterior using Kullback–Leibler (KL) divergence, learning to model more object information with limited context data and generalize to new scenes. Detailed derivations are provided in Appendix~\ref{supp:elbo}.

% \noindent{\textbf{Empirical Objective.}} 
For the geometric bases $\mathbf{B}_C$, we regularize the spatial shape of the context geometric bases to be closer to that of the target one $\mathbf{B}_T$ by introducing a KL divergence. 
Therefore, given the above ELBO, our objective function consists of three parts: a reconstruction loss (MSE loss), KL divergences for hierarchical latent variables, and a KL divergence for the geometric bases. 
%constraint for matching the two sets of Gaussian basis to ensure the basis obtained from context is as close to the one from the target. 
The empirical objective for the proposed \method{} is formulated as:
\begin{equation}
\begin{aligned}
& \mathcal{L}_{\text{\method{}}}  =  ||y - y'||^2_2 + \alpha \cdot \big(  D_{\text{KL}} [p(\mathbf{z}_o|{\bf{B}}_C)|q(\mathbf{z}_o|{\bf{B}}_T)] \\
    & + D_{\text{KL}}[p(\mathbf{z}_r|\mathbf{z}_o,{\bf{B}}_C)|q(\mathbf{z}_r|\mathbf{z}_o,{\bf{B}}_T)] \big) + \beta \cdot D_{\text{KL}}[{\bf{B}}_C, {\bf{B}}_T],
\end{aligned}
\end{equation}
where $y'$ is the prediction. $\alpha$ and $\beta$ are hyperparameters to balance the three parts of the objective. The KL divergence on ${\bf{B}}_C, {\bf{B}}_T$ is to align the spatial location and the shape of two sets of bases. 

% +++++++++++++

% \noindent 
% \textbf{Neural Fields.}
% % \zx{First introduce NeRF (with problem definition and notations) and its disadvantages of inefficient inference, then say what we will do to avoid this problem by NP?} 


% In general, training a NeRF requires overfitting each scene, which is time-consuming. Hence, how to leverage the observation for generalization on the new scene remains a problem. As each INR is a function of a data sample, the problem can be viewed as estimating the distribution of functions. This motivates us to use the Neural Process (NP) in this problem. 
 

% \noindent {\textbf{Neural Process.}} Neural Process~\cite{garnelo2018neural} parameterizes the distribution of functions. Given the context set comprising of the observation $X$ and the corresponding labels $Y$, $D_C = (X_C, Y_C) := (\mathbf{x}_i, \mathbf{y}_{i})_{i\in C} $. The aim of NP is to learn a mapping function from the target points $X_T$ to the target labels $Y_T$,  $D_T = (X_T, Y_T) := (\mathbf{x}_i, \mathbf{y}_{i})_{i\in T} $. The conditional distribution of target points is:
% \begin{equation}
%     p_{\phi}(Y_T|X_T,D_C) = \prod_{\mathbf{x}, \mathbf{y}\in D_{T}} \mathcal{N}(\mathbf{y};\mu_{\mathbf{y}}(\mathbf{x},D_c), \sigma^2_{\mathbf{y}}(\mathbf{x},D_c)).
% \end{equation}

% \begin{equation}
%     p_{\phi}(Y_T|X_T, \mathbf{z}) = \prod_{\mathbf{x}, \mathbf{y}\in D_{T}} \mathcal{N}(\mathbf{y};\mu_{\mathbf{y}}(\mathbf{z}, X_T,D_c), \sigma^2_{\mathbf{y}}(\mathbf{z}, X_T,D_c)),
% \end{equation}
% where $\mathbf{z} \sim p_{\theta}(\mathbf{z|X_T,D_C})$. Using NP can efficiently leverage the limited context/observation to infer the function of INR for the target from a probabilistic perspective. It also can incorporate uncertainty estimation for the unseen view. This is reasonable as the value in the unseen target location should not be deterministic. 

%\zx{advantages of NP? incorporating uncertainty for limited context information, which is suitable for reconstruction tasks?}







% \begin{align}
%     p(\mathbf{y}|\mathbf{x}, I) & = \int_{g} \int_{r}  p(\mathbf{y}, g, r |\mathbf{x}, I) \mathrm{d}g  \mathrm{d}r \\
%     &=  \int_{g} \int_{r}  p(\mathbf{y}| g, r) p(g, r | \mathbf{x}, I) \mathrm{d}g  \mathrm{d}r \\
%     % &= \int_{g} \int_{r} \int_{B} p_{\theta_1}(\mathbf{y}| g, r) p_{\theta_2}(g, r | B) p_{\theta_3}(B|\mathbf{x}, I) \mathrm{d}g  \mathrm{d}r \mathrm{d}B 
%     &= \int_{g} \int_{r}  p_{\theta_1}(\mathbf{y}| g, r) p_{\theta_2}(g, r | B) p_{\theta_3}(B|\mathbf{x}, I) \mathrm{d}g  \mathrm{d}r 
% \end{align}


%\subsection{Gaussian Basis for INR}
%As shown in Fig.~\ref{fig:framework}, 


%\subsection{Hierarchical Neural Process for INR}









==> Sections/3method.tex <==

\subsection{Preliminary}

\textcolor{red}{start with 3D, make it clear on 3D. function. }

\noindent 
\textbf{Neural Fields.}
% \zx{First introduce NeRF (with problem definition and notations) and its disadvantages of inefficient inference, then say what we will do to avoid this problem by NP?} 
The implicit neural field defines a continuous function $f_\theta : \mathbf{x} \mapsto \mathbf{y}$ from spatial coordinates to arbitrary signals, where $\theta$ is the function weights, $X\in \mathbb{R}^c$ is the coordinates, and $Y\in \mathbb{R}^d$ is the target signal. In neural radiance field (NeRF)~\cite{mildenhall2021nerf}, the 3D locations with view direction $v$ are mapped to 4D tuples of the densities and RBG values. However, training a NeRF requires overfitting each scene, which is time-consuming. Hence, how to leverage the observation for generalization on the new scene remains a problem. As each INR is a function of a data sample, the problem can be viewed as estimating the distribution of functions. This motivates us to use the Neural Process (NP) in this problem. 
 



\noindent {\textbf{Neural Process.}} Neural Process~\cite{garnelo2018neural} parameterizes the distribution of functions. Given the context set comprising of the observation $X$ and the corresponding labels $Y$, $D_C = (X_C, Y_C) := (\mathbf{x}_i, \mathbf{y}_{i})_{i\in C} $. The aim of NP is to learn a mapping function from the target points $X_T$ to the target labels $Y_T$,  $D_T = (X_T, Y_T) := (\mathbf{x}_i, \mathbf{y}_{i})_{i\in T} $. The conditional distribution of target points is:
\begin{equation}
    p_{\phi}(Y_T|X_T,D_C) = \prod_{\mathbf{x}, \mathbf{y}\in D_{T}} \mathcal{N}(\mathbf{y};\mu_{\mathbf{y}}(\mathbf{x},D_c), \sigma^2_{\mathbf{y}}(\mathbf{x},D_c)).
\end{equation}

\begin{equation}
    p_{\phi}(Y_T|X_T, \mathbf{z}) = \prod_{\mathbf{x}, \mathbf{y}\in D_{T}} \mathcal{N}(\mathbf{y};\mu_{\mathbf{y}}(\mathbf{z}, X_T,D_c), \sigma^2_{\mathbf{y}}(\mathbf{z}, X_T,D_c)),
\end{equation}
where $\mathbf{z} \sim p_{\theta}(\mathbf{z|X_T,D_C})$. Using NP can efficiently leverage the limited context/observation to infer the function of INR for the target from a probabilistic perspective. It also can incorporate uncertainty estimation for the unseen view. This is reasonable as the value in the unseen target location should not be deterministic. 

%\zx{advantages of NP? incorporating uncertainty for limited context information, which is suitable for reconstruction tasks?}


\subsection{$N^2\text{P}$}
\textcolor{red}{Name: use $N^2\text{P}$ temporarily.}

\begin{figure}[h]
  \centering
  \includegraphics[width=0.99\textwidth]{Figures/framework_draft.pdf} % Adjust the size and filename as needed
  \caption{Framework.} % Caption for the figure
  \label{fig:framework}
\end{figure}

To improve the generalization ability and achieve efficient inference on new scenes of Neural Field methods, we propose to learn to infer specific model parameters for each scene by Neural Processes.
\zx{Advantages}
In the following, we use NeRF generalization to illustrate the proposed method.  In NeRF generalization, a few views (one or two) of images $I_c$ and its corresponding camera pose $\mathbf{p}$ serve as the context information. 
%We represent each location in this scene by aggregating these Gaussians basis based on the radial basis function (RBF). 
Then, based on the context information, the task is to estimate an implicit function that can be used to infer the target for unseen views.

The proposed GP-INR framework assumes a space composed of a set of Gaussian bases that encodes the spatial location and semantic information of a scene. Initially, GP-INR predicts a Gaussian basis $B_C$ from the observed context. Similar to the recent advances in implicit neural fields (e.g., Neurbf~\cite{chen2023neurbf}), at arbitrary new locations $X_T \in \mathbb{R}^{N\times P\times 3}$, we aggregate the Gaussians to form a new representation of this location $X'_C$ via the radial basis function (RBF). By averaging the representations both globally and locally along rays, we obtain a global latent $g_C$ and a ray-specific latent $r_C$ to modulate an MLP for predicting the implicit neural field. During training, with the target view and image $I_T$ also provided, we perform the same procedures for $I_T$ and align latent variables from both the context and target. For simplicity, in the following, we will use $I_C$ as an example to illustrate. 

NerF: $F: (x,y,z,\theta,\phi) \mapsto (c,\sigma)$. 

Context set (camera pose and image rbg level): 
\begin{align}
\tilde{X}_c:&= \{ \tilde{x}_i \}_{i=1}^{N_c}, \tilde{x}_i \in \mathbb{R}^{6} (\text{ray-o}, \text{ray-d})\\
\tilde{Y}_c:&= \{ \tilde{y}_i \}_{i=1}^{N_c}, \tilde{y}_i \in \mathbb{R}^{3} (\text{RGB})
\end{align}

Target set (3d coordinates and 3d rbg with density level):

$x_i$ is a set of 3D points corresponding to a specific ray direction. 
\begin{align}
X_t:&= \{ x_i \}_{i=1}^{N_t}, x_i \in \mathbb{R}^{P\times3} (\text{sampled 3D points})\\
Y_t:&= \{ y_i \}_{i=1}^{N_t}, y_i \in \mathbb{R}^{P\times4} (c,\sigma)
\end{align}

\begin{align}
    p(Y_t|X_t, \tilde{X}_c, \tilde{Y}_c) & = p(Y_t|X_t,B_c)p(B_c|\tilde{X}_c, \tilde{Y}_c) \\
    &= \Pi_{i=1}^{N_t} p(y_i|x_i, g, r_i, B_c) p(r_i|g, x_i) p(g|B_c, X_t) p(B_c|\tilde{X}_c, \tilde{Y}_c)
\end{align}

\begin{align}
    p(Y_t|X_t, \tilde{X}_c, \tilde{Y}_c) & \approx p(Y_t|X_t,B_c) \\
    &= \Pi_{i=1}^{N_t} p(y_i|x_i, g, r_i, B_c) p(r_i|g, x_i) p(g|B_c, X_t)
\end{align}

Question: 
\textcolor{red}{Does the gap between $(\tilde{X},\tilde{Y})$ and $(X,Y)$ support our motivation of using basis for NP? Motivation: as there is an information gap between $(\tilde{X},\tilde{Y})$ as $(X)$ is sampled from $(\tilde{X}$, Y can be seen as sampled from $\tilde{Y}$ ($Y$ is discrete, $\tilde{Y}$ is the integration result over all the ray), we introduce a Gaussian basis to encode the geometry information in the space. The Gaussian basis with radial basis function provides a continuous way of representing spatial location to reduce the information loss. 
}
\begin{align}
    p(\mathbf{y}|\mathbf{x}, I) & = \int_{g} \int_{r}  p(\mathbf{y}, g, r |\mathbf{x}, I) \mathrm{d}g  \mathrm{d}r \\
    &=  \int_{g} \int_{r}  p(\mathbf{y}| g, r) p(g, r | \mathbf{x}, I) \mathrm{d}g  \mathrm{d}r \\
    % &= \int_{g} \int_{r} \int_{B} p_{\theta_1}(\mathbf{y}| g, r) p_{\theta_2}(g, r | B) p_{\theta_3}(B|\mathbf{x}, I) \mathrm{d}g  \mathrm{d}r \mathrm{d}B 
    &= \int_{g} \int_{r}  p_{\theta_1}(\mathbf{y}| g, r) p_{\theta_2}(g, r | B) p_{\theta_3}(B|\mathbf{x}, I) \mathrm{d}g  \mathrm{d}r 
\end{align}


\subsection{Gaussian Basis for INR}
%As shown in Fig.~\ref{fig:framework}, 
\noindent {\textbf{Gaussian Basis.}} When a human sees a view of a scene (context image), the posterior knowledge about the color and spatial location of the scene is revealed. We encode this posterior knowledge as a form of Gaussian basis set, which is spanned in the space. 
Given an image $I_C \in \mathbb{R}^{H\times W \times 3}$, a visual self-attention module first produces a $M\times D$ tokens with $M$ as the number of visual tokens, and $D$ as the hidden dimension. The number of Gaussians we use equals to the number of tokens $M$. That being said, we use one MLP to predict the spatial shape of Gaussians, including the mean $\mu$, as well as the rotation and scaling parameters for producing the covariance matrix $\Sigma$, and one MLP to produce the corresponding latent representations $\omega \in \mathbb{R}^{M \times D} $. The covariance matrix is obtained by:
\begin{equation}
    \Sigma = RSS^TR^T,
    \label{eq:cov-matrix}
\end{equation}
where $R\in \mathbb{R}^{3\times3}$ is the rotation matrix, and $S \in \mathbb{R}^3$ is the scaling matrix. 

By using the Gaussian basis set, we are able to 1). aggregate the locality information for the input which is similar to NeuRBF~\cite{chen2023neurbf}; 2). generate a global latent variable of the scene and location-specific latent variables for modulating the implicit neural field for generalization purposes.

\noindent {\textbf{Aggregation.}} We represent each spatial location in the scene by considering the scene information. For each spatial location, we aggregate the locality information to the current location. Note that, in the classical INR, the locality latents are learned by overfitting, while ours is based on the predicted Gaussian basis. For arbitrary target locations $X_t$, we employ a Gaussian radial basis function to aggregate the information from the predicted Gaussian basis and obtain a new representation of this location $X'_C$:
\begin{equation}
    X'_C = \text{MLP}(\sum_i^{M} \varphi(x, \mu_i, \Sigma_i)\omega_i)
\end{equation}

\begin{equation}
    \varphi(x, \mu_i, \Sigma_i) = \exp(-\frac{1}{2} (x-\mu_i)^T\Sigma_i^{-1}(x-\mu_i))
\end{equation}

\subsection{Hierarchical Neural Process for INR}


\noindent{{\textbf{Hierarchical Neural Process.}}} Based on the re-represented spatial representation, we perform a hierarchical neural process. Our latent variables consist of two parts, the global variable $g_C$ and the ray or location-specific variables $r_C$. The formulation of NP is given by:
% \begin{equation}
%     p(\mathbf{y}|\mathbf{x}, I_C) = \int p(\mathbf{y}|\mathbf{x}, g_C, r_C) p(g_C, r_C|\mathbf{x}, I_C). 
% \end{equation}

\begin{align}
    p(\mathbf{y}|\mathbf{x}, I) = \int_{g} \int_{r}  p_{\theta_1}(\mathbf{y}| g, r) p_{\theta_2}(g, r | B) p_{\theta_3}(B|\mathbf{x}, I) \mathrm{d}g  \mathrm{d}r 
\end{align}

\textcolor{red}{To be discussed how to write}

\noindent{\textbf{ELBO.}} $p_{\theta_3}$ is a deterministic function, and $p_{\theta_1}$ is the decoder, which is the modulated implicit function in our case. Hence, we are interested in the posterior of $p_{\theta_2}(\mathbf{g}, \mathbf{r} | B)$. We want to align the posteriors from the context and target during training. 

\begin{align}
    \log p(\mathbf{y_t}|\mathbf{x_t}, I_c) = \mathbb{E}_{q(g_c,r_c|\mathbf{x_t}, I_t)} 
\end{align}


We parameterize $p(g_C, r_C|\mathbf{x}, I_C)$ as hierarchical latent variables. We first aggregate globally to obtain $p(g_C)$. The local variable $p(r_C)$ is obtained by firstly aggregating ray-wisely and then updating it through a transformer together with the global vector sampled from $p(g_C)$. 



\noindent {\textbf{Global Variable.}} We use a global latent variable $g$ to describe the scene. In NeRF reconstruction, points are sampled from rays, leading to the target points $X_T\in \mathbb{R}^{N\times P\times 3}$, where $N$ is the number of rays, and $P$ is the number of points sampled from each ray. To obtain the global variable, we average over all points and pass through an MLP. 
\begin{equation}
    g_C = [\mu^c_g, \sigma^c_g] = \text{MLP}(\frac{1}{N\times P}\sum_j^{N\times P}(X'_C)[j]),
\end{equation}
where $\mu^c_g$ and $\sigma^c_g$ are the mean and variance of global variables, respectively. We sample global latent vector by $\hat{g}_c \sim \mathcal{N}(\mu^c_g, \sigma^c_g)$. 


\noindent {\textbf{Location-specific Variable.}} Moreover, modulating the implicit function through the global variable lacks the local detail information. Hence, we propose a spatial location-specific modulation (ray-specific in NerF). We infer a ray-specific variable $r_c$ by first aggregating the feature ray-wisely:
\begin{equation}
    r'_c = \text{MLP}(\frac{1}{ P}\sum_j^{P}(X'_C)[j])
\end{equation}


Then, we perform a hierarchical formulation by incorporating the global variable to obtain the ray-specific variable. This enables us to design the latent variable in a hierarchical structure, which is rational as it learns the scene coarse-to-fine. $r_c$ is obtained by feeding $r'_c$ together with the sampled $\hat{g}_c$ into a Transformer: 
\begin{equation}
    r_c = [\mu^c_r, \sigma^c_r] = \text{Transformer}([\hat{g}_c; \hat{r}_C]),
\end{equation}
where $\mu^r_g$ and $\sigma^r_g$ are the mean and variance of global variables, respectively. Details of the Transformer architecture are given in the Appendix. 


\noindent {\textbf{Modulation.}} The latent variable to modulate the MLP is $[g_c;r_c]$
The modulated MLP layer used in our paper is similar to the style \textit{modulation} in ~\cite{guo2023versatile}. Essentially, we predict a style vector $s\in \mathbb{R}^{d_{in}}$ to multiply or scale the weight matrix of an MLP, $W \in \mathbb{R}^{d_{in} \times d_{out}}$.




\noindent{\textbf{Loss.}} Our loss consists of three parts, the regression loss $L_{\text{MSE}}$, the KL divergence between latent variables from context and target, and the constraint for matching the two sets of Gaussian basis to ensure the basis obtained from context is as close to the one from the target. 

\begin{equation}
    L_{\text{MSE}} = ||y - y'||^2_2 + \alpha D_{\text{KL}}(p(g_C|B_C)|q(g_T|B_T)) + \beta \text{KL}(B_C, B_T)
\end{equation}
where $y'$ is the prediction, $D_{\text{KL}}$ is the KL divergence, $\alpha$ and $\beta$ are two weighting hyperparameters. 



==> Sections/4experiments.tex <==

% We evaluate the proposed \method{} on different tasks.
% In Sec.~\ref{sec:nerf-results}, we demonstrate the performance on novel view synthesis for 3D scenes. 
% Further, we show the method can also perform competitively on the 2D image regression task, as well as image completion in Sec.~\ref{sec:image-regression}, although it is originally designed for 3D view synthesis.
% Last, we perform ablation studies in Sec.~\ref{sec:abl-study}. 

\noindent{\textbf{Baselines.}}
%\str{Explain why meta-learning is the type of baseline we want here.}
We compare \method{} with three recent probabilistic INR generalization methods: NeRF-VAE~\citep{kosiorek2021nerf}, PONP~\citep{gu2023generalizable} and VNP~\citep{guo2023versatile} on ShapeNet novel view synthesis and image regression tasks.
PONP~\citep{gu2023generalizable} and VNP~\citep{guo2023versatile} also rely on Neural Processes, however, they neglect structure information and the probabilistic interaction between 3D functions and 2D partial observations. Additionally, we choose two previous well-known deterministic INR generalization approaches, LearnInit~\citep{tancik2021learned} and  TransINR~\citep{chen2022transformers} as our baselines. Moreover, to demonstrate the flexibility of our method and its ability to handle complex scenes, we integrate \method{} with GNT~\citep{wang2022attention} and conduct experiments on the NeRF Synthetic dataset~\citep{mildenhall2021nerf}. \textcolor{blue}{In addition, we demonstrate our method is also effective for 1-D signals in the Appendix.}


% We choose two previous well-known deterministic INR generalization approaches, LearnInit~\citep{tancik2021learned} and  TransINR~\citep{chen2022transformers} as our baselines. We use the self-attention module similar to TransINR to extract features from the context set.
% Additionally, we compare with three recent probabilistic INR generalization methods: NeRF-VAE~\citep{kosiorek2021nerf}, PONP~\citep{gu2023generalizable} and VNP~\citep{guo2023versatile}.
% PONP~\citep{gu2023generalizable} and VNP~\citep{guo2023versatile} also rely on Neural Processes, however, they neglect structure information and the probabilstic interaction between 3D functions and 2D partial observations.


\subsection{Novel View Synthesis}
\label{sec:nerf-results}

% \noindent{\textbf{Setup.}} We perform the 3D novel view synthesis task on ShapeNet~\citep{chang2015shapenet} objects. Following previous works' setup, the dataset consists of objects from three ShapeNet categories: chairs, cars, and lamps. For each 3D object, 25 views of size $128 \times 128$ images are generated from viewpoints randomly selected on a sphere. The objects in each category are divided into training and testing sets, with each training object consisting of 25 views with known camera poses. During testing, a random input view is sampled to evaluate the performance of the novel view synthesis. Following the setting from previous methods, we focus on the single-view (1 shot) and 2-views (2 shot) versions of the task, where single-view or two-view images with their corresponding camera rays are provided as the context set.
\noindent{\textbf{ShapeNet.}} We perform the 3D novel view synthesis task on ShapeNet~\citep{chang2015shapenet} objects. Following previous works' setup~\citep{tancik2021learned}, the dataset consists of objects from three ShapeNet categories: chairs, cars, and lamps. For each 3D object, 25 views of size \(128 \times 128\) images are generated from viewpoints randomly selected on a sphere. The objects in each category are divided into training and testing sets, with each training object consisting of 25 views with known camera poses. At test time, a random input view is sampled to evaluate the performance of the novel view synthesis. Following the setting of previous methods~\citep{chen2022transformers}, we focus on the single-view (1-shot) and 2-view (2-shot) versions of the task, where one or two images with their corresponding camera rays are provided as the context.


% \noindent{\textbf{Implementation Details.}} 
% %We use the visual tokenizer and self-attention modules as TransINR~\citep{chen2022transformers} and VNP~\citep{guo2023versatile}. 
% Our context input is the concatenation of a set of camera rays and the corresponding image pixels from a few views (one or two),
% %the context image and the corresponding ray maps %\str{What is a ray map?}, 
% which are then split into different visual tokens. We use the same patch size $8\times8$ as TransINR~\citep{chen2022transformers} and VNP~\citep{guo2023versatile}, which gives us 256 tokens. 
% Then, a linear layer and a self-attention module are used to project each token into a 512-dimension vector. Based on the 256 tokens, we predict 256 Gaussian bases by two MLP modules. Specifically, one MLP with 2 linear layers is used to map the tokens into a 10-dimension vector, which includes 3-dimension Gaussian centers a 3-dimension vector for constructing the scaling matrix, and a 4-dimension vector for quaternions parameters of the rotation matrix. Both the scaling matrix and rotation matrix are used to build the $3\times 3$ covariance matrix. This procedure is similar to Gaussian construction in the 3D Gassian Splatting~\citep{kerbl20233d}. Details are provided in the Appendix. Another MLP is used to estimate the latent representation of each Gaussian basis. Here, we simply use 32-dimension for each Gaussian basis. 
% Note that using more views as the context set will increase the number of Gaussian basis accordingly, which enriches the ability of describing the geometry of the space. 


\begin{table*}[t]
    \centering
    \caption{\textbf{Qualitative comparison (PSNR) on novel view synthesis of ShapeNet objects.} \method{} consistently outperforms baselines across all categories with both 1-view and 2-view context.}
    \begin{tabular}{lccccc}
        \toprule
        Method & Views & Car & Lamps & Chairs & Average \\
        \midrule
        Learn Init~\citep{tancik2021learned}  & 25 & 22.80 & 22.35 & 18.85 & 21.33 \\
        \midrule
        Tran-INR~\citep{chen2022transformers}  & 1 & 23.78 & 22.76 & 19.66 & 22.07 \\
        NeRF-VAE~\citep{kosiorek2021nerf}  & 1 & 21.79 & 21.58 & 17.15 & 20.17 \\
        PONP~\citep{gu2023generalizable}  & 1 & 24.17 & 22.78 & 19.48 & 22.14 \\
        VNP~\citep{guo2023versatile}  & 1 & 24.21 & 24.10 & 19.54 & 22.62 \\
        \rowcolor{lightblue}
        \textbf{\method{}} (Ours) & 1 & \textbf{25.13} & \textbf{24.59} & \textbf{20.74} & \textbf{23.49} \\
        \midrule
        Tran-INR~\citep{chen2022transformers}  & 2 & 25.45 & 23.11 & 21.13 & 23.27 \\
        PONP~\citep{gu2023generalizable}  & 2 & 25.98 & 23.28 & 19.48 & 22.91 \\
        \rowcolor{lightblue}
        \textbf{\method{}} (Ours) & 2 & \textbf{26.39} & \textbf{25.32} & \textbf{22.68} & \textbf{24.80} \\
        \bottomrule
    \end{tabular}
    \label{tab:nerf-psnr}
    \vspace{-2mm}
\end{table*}

\begin{figure*}[t]
  \centering
  \includegraphics[width=1\textwidth]{Figures/nerf-results-new.pdf} % Adjust the size and filename as needed
  \vspace{-6mm}  \caption{\textbf{Qualitative results of the proposed \method{} on novel view synthesis of ShapeNet objects.} Both 1-view (top) and 2-view (bottom) context results are presented.} % Caption for the figure
  \label{fig:nerf-visualization}
  \vspace{-3mm}
\end{figure*}

\noindent{\textbf{Implementation Details.}} Our context input is the concatenation of a set of camera rays and the corresponding image pixels from one or two views, which are then split into different visual tokens. We use the same patch size \(8 \times 8\) as TransINR~\citep{chen2022transformers} and VNP~\citep{guo2023versatile}, resulting in 256 tokens. A linear layer and a self-attention module project each token into a 512-dimensional vector. Based on the 256 tokens, we predict 256 geometric bases using two MLP modules: one for 3D Gaussian distribution parameters and the other for the latent representation (32 dimensions).
% \wy{Can be removed to appendix: Specifically, one MLP with 2 linear layers maps the tokens into a 10-dimensional vector, which includes 3-dimensional Gaussian centers, a 3-dimensional vector for constructing the scaling matrix, and a 4-dimensional vector for quaternion parameters of the rotation matrix. Both the scaling matrix and rotation matrix are used to build the \(3 \times 3\) covariance matrix. This procedure is similar to Gaussian construction in the 3D Gaussian Splatting~\citep{kerbl20233d}.} 
%We use one MLP to predict Gaussian basis parameters, which is detailed in the Appendix. Another MLP estimates the latent representation of each Gaussian basis, using a 32-dimensional vector for each Gaussian basis. 
More details are given in Appendix~\ref{supp:gaussian}. 
%Using more views as the context set increases the number of geometric base accordingly, enriching the ability to describe the geometry of the space.
% To have a fair comparison with baseline methods, we report the results of using $8\times 8$ patch size. \str{What do you mean here? Other baselines also use 8x8 patches? If yes, say that.}
We obtain the object-specific and ray-specific modulating vectors (both are 512 dimensions) based on the geometric base. Our NeRF function consists of four layers, including two modulated layers and two shared layers. %\str{This can also be better written. The terminology is not consisten, what is the global and local-raywise modulate vectors? We not really use that words before.}

\noindent{\textbf{Quantitative Results.}} The quantitative comparison in terms of Peak Signal-to-Noise Ratio (PSNR) is presented in Table~\ref{tab:nerf-psnr}. The proposed \method{} consistently outperforms all other baselines across all three categories by a significant margin. On average, \method{} exceeds the previous NP-based method, VNP~\citep{guo2023versatile}, by 0.87 PSNR, %(23.49 vs. 22.62), 
indicating that the proposed geometric bases and probabilistic hierarchical modulation result in better generalization ability. Moreover, with two views of context information, \method{}'s performance improves significantly by around $1$ PSNR. This improvement is expected, as the richer geometric bases information allows for a better representation of the 3D space, leading to improved object-specific and ray-specific latent variables. % to modulate the MLP.




{\noindent {\textbf{Qualitative Results.}}
In Fig.~\ref{fig:nerf-visualization}, we visualize the results of \method{} on novel view synthesis of ShapeNet objects.
\method{} can infer object-specific radiance fields and render high-quality 2D images of the objects from novel camera views, even with only 1 or 2 views as context. More results and comparisons with other VNP are provided in Appendix~\ref{supp:more-results}.}


\textcolor{blue}{\noindent \textbf{Comparison with More SOTAs on NeRF Synthetic.} To illustrate the flexibility and advantages of our proposed method, we evaluate it on the NeRF Synthetic dataset~\citep{mildenhall2021nerf} against recent state-of-the-art methods, including GNT~\citep{wang2022attention}, MatchNeRF~\citep{chen2023explicit}, and GeFu~\citep{liu2024geometry}. For a fair comparison, we use the same encoder and NeRF network architecture while integrating our probabilistic framework into GNT. Following GeFu, we assess performance in 2-view and 3-view settings. As shown in Table~\ref{tab:comparison-gnt}, our method surpasses GeFu by approximately 1 PSNR in the 3-view setting, validating the effectiveness of our probabilistic framework and geometric bases.}

\textcolor{blue}{We also consider a challenging 1-view setting to examine the model’s robustness under extremely limited context. Both Table~\ref{tab:comparison-gnt} and Figure~\ref{fig:1-view-compare} indicate that our method can still reconstruct novel views effectively, whereas GNT fails to do so. Furthermore, we test cross-category generalization for our model and GNT without retraining, training on the \texttt{drums} category and evaluating on \texttt{lego}. As shown in Figure~\ref{fig:cross-category}, our method leverages the available context information more effectively, producing higher-quality generations with superior color fidelity compared to GNT. Additional details are provided in Appendix~\ref{sec:compare_gnt}.}


\begin{table}[htbp]
\centering
\resizebox{\columnwidth}{!}{ % Resize the table to fit within the column width
\begin{tabular}{lcccc}
\toprule
\textbf{Models} & \textbf{\# Views} & \textbf{PSNR ($\uparrow$)} & \textbf{SSIM ($\uparrow$)} &  \textbf{LPIPS ($\downarrow$)}\\ 
\midrule
GNT  & 1 & 10.25 & 0.583 & 0.496\\ 
GeomNP & 1 & \textbf{20.07} & \textbf{0.815} & \textbf{0.208} \\ 
\midrule
GNT & 2 & 23.47 &0.877 &0.151 \\ 
MatchNeRF & 2 &20.57 & 0.864 &0.200  \\ 
GeFu & 2 & 25.30 &0.939 &0.082  \\ 
GeomNP & 2 &  &  &  \\ 
\midrule
GNT & 3 &  25.80 & 0.905 & 0.104 \\ 
MatchNeRF & 3 & 23.20 & 0.897 & 0.164  \\ 
GeFu & 3 &  26.99 & \textbf{0.952} & 0.070  \\ 
GeomNP & 3 & \textbf{27.85} & 0.948 & \textbf{0.068} \\ 
\bottomrule
\end{tabular}
}
\caption{Performance comparison of different models with varying numbers of context views.}
\label{tab:comparison-gnt}
\end{table}





\begin{table}[htbp]
    \centering
    \begin{tabular}{lcc}
        \toprule
                 & CelebA & Imagenette \\ \midrule
        Learned Init \citep{tancik2021learned} & 30.37  & 27.07       \\
        TransINR~\citep{chen2022transformers}  & 31.96  & 29.01       \\ 
        \rowcolor{lightblue}
        \textbf{\method{} (Ours)}         & \textbf{33.41}  & \textbf{29.82}      \\ 
        \bottomrule
    \end{tabular}
    \caption{Quantitative results. \method{} outperforms baseline methods consistently on both datasets.}
    \label{tab:image-regression}
\end{table}


\begin{figure}[htbp]
    \centering
    \begin{minipage}[b]{0.49\textwidth} 
        \includegraphics[width=\textwidth]{Figures/image-regression0.pdf} % Adjust filename as needed
        \caption{\textbf{Visualizations of image regression results} on CelebA (left) and Imagenette (right).}
        \label{fig:visualization-image-regression}
    \end{minipage}
\end{figure}


% \begin{figure*}[htbp]
%     \centering
%     \begin{subtable}[b]{151.2pt} 
%     % \vspace{-6mm}
%     \begin{tabular}{lcc}
%     \toprule
%                  & CelebA & Imagenette \\ \midrule
%     Learned Init \citep{tancik2021learned} & 30.37  & 27.07       \\
%     TransINR~\citep{chen2022transformers}         & 31.96  & 29.01       \\ 
%     % \hline
%     \rowcolor{lightblue}
%     \textbf{\method{}} (Ours)         & \textbf{33.41}  & \textbf{29.82}      \\ 
%     \bottomrule
%     \end{tabular}
%     \caption{Quantitative results. \method{} outperforms baseline methods consistently on both datasets.}
%     \label{tab:image-regression}
%     \end{subtable} \hfill
%     \begin{subtable}[b]{151.2pt} 
%     \includegraphics[width=\textwidth]{Figures/image-regression0.pdf} % Adjust the size and filename as needed
%     \caption{Visualizations on CelebA (left) and Imagenette (right), respectively.} % Caption for the figure
%     \label{fig:visualization-image-regression}
% \end{subtable}
% % \vspace{-2mm}
% \caption{\textbf{Quantitative results and visualizations} of image regression on CelebA and Imagenette.}
% \vspace{-3mm}
% \end{figure*}





% \begin{figure}[t]
%     \centering
%     \begin{subtable}[b]{0.42\textwidth}
%     % \vspace{-6mm}
%     \begin{tabular}{lcc}
%     \toprule
%                  & CelebA & Imagenette \\ \midrule
%     Learned Init \citep{tancik2021learned} & 30.37  & 27.07       \\
%     TransINR~\citep{chen2022transformers}         & 31.96  & 29.01       \\ 
%     % \hline
%     \rowcolor{lightblue}
%     \method{} (Ours)         & \textbf{33.41}  & \textbf{29.82}      \\ 
%     \bottomrule
%     \end{tabular}
%     \caption{Quantitative results. \method{} outperforms baseline methods consistently on both datasets.}
%     \label{tab:image-regression}
%     \end{subtable} \hfill
%     \begin{subtable}[b]{0.54\textwidth}
%     \includegraphics[width=\textwidth]{Figures/image-regression0.pdf} % Adjust the size and filename as needed
%     \caption{Visualizations on CelebA (left) and Imagenette (right), respectively.} % Caption for the figure
%     \label{fig:visualization-image-regression}
% \end{subtable}
% % \vspace{-2mm}
% \caption{\textbf{Quantitative results and visualizations} of image regression on CelebA and Imagenette.}
% \vspace{-3mm}
% \end{figure}



\subsection{Image Regression}
\label{sec:image-regression}


\noindent{\textbf{Setup.}} Our method is flexible to different signals and can also be seamlessly applied to 2D signals. Here, we evaluate our method on the image regression task, a common task for evaluating INRs' capacity of representing a signal~\citep{tancik2021learned,sitzmann2020implicit}. 
We employ two real-world image datasets as used in previous works~\citep{chen2022transformers,tancik2021learned,gu2023generalizable}. The CelebA dataset~\citep{liu2015deep} encompasses approximately 202,000 images of celebrities, partitioned into training (162,000 images), validation (20,000 images), and test (20,000 images) sets. The Imagenette dataset~\citep{imagenette}, a curated subset comprising 10 classes from the 1,000 classes in ImageNet~\citep{deng2009imagenet}, consists of roughly 9,000 training images and 4,000 testing images. In order to compare with previous methods, we conduct image regression experiments. The context set is an image and the task is to learn an implicit function that regresses the image pixels well. % in terms of PSNR.
%\str{What is the point of image regresssion when the image itself is used as context? Why not just copy the context??}
%\str{The following is a bit strante, is this still image regression? Why not have a separate section?}
%\str{Is Image Regression the standard name for this task?}


\noindent{\textbf{Implementation Details.}} 
Following TransINR~\citep{chen2022transformers}, we resize each image into $178\times 178$, and use patch size 9 for the tokenizer. The self-attention module remains the same as the one in the NeRF experiments (Sec. \ref{sec:nerf-results}). For the Gaussian bases, we predict the 2D Gaussians instead of the 3D. 
The hierarchical latent variables are inferred in image-level and pixel-level. 
%The self-attention and global variable remain the same as the one in the NeRF experiments. %We do not use the pixel variable modulation for the computation concern. However, our method still has competitive performance.   

% \begin{table}[t]
% \centering
% \vspace{-6mm}
% \caption{Quantitative results of image regression.}
% \label{tab:image-regression}
% \begin{tabular}{lcc}
% \toprule
%              & CelebA & Imagenette \\ \midrule
% Learned Init \citep{tancik2021learned} & 30.37  & 27.07       \\
% TransINR~\citep{chen2022transformers}         & 31.96  & 29.01       \\ 
% \hline
% \method{} (Ours)         & \textbf{33.41}  & \textbf{29.82}      \\ 
% \bottomrule
% \end{tabular}
% \end{table}



\noindent{\textbf{Results.}} The quantitative comparison of \method{} for representing the 2D image signals is presented in Table~\ref{tab:image-regression}. \method{} outperforms the baseline methods on both CelebA and Imagenette datasets significantly, showing better generalization ability and representation capacity than baselines. 
%Note that the Imagenette is a more diverse dataset than the CelebA. The better performance shows that. 
Fig.~\ref{fig:visualization-image-regression} shows the ability of \method{} to recover the high-frequency details for image regression.
%regress the image closely to the ground truth, indicating the capability of capturing the detailed texture information. 





%, implying good capability of .



% \begin{figure}[t]
%   \centering
%   \includegraphics[width=0.9\textwidth]{Figures/image-regression-vis.pdf} % Adjust the size and filename as needed
%   \caption{Image regression visualization on CelebA and Imagenette, respectively. Left: Ground truth; Right: Prediction.} % Caption for the figure
%   \label{fig:visualization-image-regression}
% \end{figure}



%\noindent {\textbf{Ablation study}}
\subsection{Ablations}
\label{sec:abl-study}

%\noindent

\begin{table}[htbp]
% \centering
\vspace{-4mm}
\caption{\textbf{Sensitivity to the number of geometric bases} on NeRF and image regression.}
\label{tab: ablate_basis}
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{lccccc}
\toprule
 & \multicolumn{3}{c}{\textbf{Image Regression}} & \multicolumn{2}{c}{\textbf{NeRF}} \\
 \cmidrule(lr){2-4} \cmidrule(lr){5-6}
\# Bases & 49 & 169 & 484 & 100 & 250 \\ \midrule
PSNR~($\uparrow$)    & 28.59  & 33.74   &  44.24  &  24.31 &  24.59  \\ \bottomrule
\label{table:num-gaussian}
\end{tabular}
}
\vspace{-6mm}
\end{table}
% \vspace{-2mm}
\textbf{Sensitivity to Number of Geometric Bases}.
We further analyze the sensitivity to the number of geometric bases in the CelebA image regression and Lamps NeRF tasks. 
We further analyze the sensitivity to the number of geometric bases in the CelebA image regression and Lamps NeRF tasks. 
In image regression, we resize the images to \(64 \times 64\) and use different patch sizes to construct 49, 169, and 484 bases. In the NeRF task, we keep the same setup as in Sec. \ref{sec:nerf-results} and construct 100, 250 bases. The results are provided in Table~\ref{table:num-gaussian}. With more bases, \method{} achieves better performance consistently, indicating that large numbers of geometric Gaussian bases further enrich the structure information and lead to stronger predictive functions. 
%However, beyond a certain point, specifically 169 in this experiment, the performance gains diminish. 
We choose the number of bases by balancing the performance and computational costs.





\noindent{\textbf{Importance of Hierarchical Latent Variables.}}
To demonstrate the effectiveness of the hierarchical nature of \method{} with object-specific and ray-specific latent variables for modulation, we performed an ablation study on a subset of the Lamps dataset for fast evaluation. As shown in the last four rows in Table~\ref{table:abl-np}, either object-specific or ray-specific latent variable improves the performance of neural processes, indicating the effectiveness of the specific function modulation. With both ${\bf{z}}_o$ and ${\bf{z}}_r$, the method performs best, demonstrating the importance of the hierarchical modulation by latent variables. 
In addition, the hierarchical modulation also performs well without the geometric bases.
% proposed NPs effectively provides both object-specific and ray-specific functions to capture detailed textures.
%Additionally, without all hierarchical latent variables, \method{} still remains a relatively good performance, which implies the outstanding capacity of the Gaussian basis. 

%drops by $0.5$ PSNR.
%The reason is that the same MLP is used for different scenes and novel views, while with the hierarchical Neural Process \str{TODO}.


% \begin{table}[htbp]
% \centering
% \caption{Ablation Study on a subset of the Lamps scene synthesis (PSNR). }
% \label{tab:my_label}
% \begin{tabular}{lc}
% \toprule
% %Basis & $\mathbf{z}_o$ (Object) & $\mathbf{z}_r$ (Ray) & PSNR \\
% Basis & PSNR \\ 
% %\midrule
% \midrule
% %\cmark & \xmark & \xmark &  25.98\\ 
% \xmark  & 23.06 \\ 
% %\cmark & \xmark & \cmark & 26.29\\ 
% %\cmark & \cmark & \xmark & 26.24\\ 
% \cmark  & 26.48\\ 
% \bottomrule
% \label{table:abl-basis}
% \end{tabular}
% \end{table}



\begin{table}[htbp]
\centering
\vspace{-4mm}
\caption{\textbf{Importance of geometric bases and hierarchical latent variables} on a subset of the Lamps scene synthesis (PSNR). $\mathbf{z}_o$ and $\mathbf{z}_r$ are object-specific variable and ray-specific variable, respectively.  \ymark~ and \xmark~denote whether the component joins the pipeline or not.}
%\vspace{-2mm}
%\label{tab:my_label}
\resizebox{0.25\textwidth}{!}{
\begin{tabular}{lccc}
\toprule
 $\mathbf{B}_C$ & $\mathbf{z}_o$& $\mathbf{z}_r$ & PSNR ($\uparrow$) \\ 
\midrule
\xmark & \cmark & \cmark & 23.06 \\
\cmark & \xmark & \xmark & 25.98 \\
\cmark & \cmark & \xmark & 26.24\\ 
\cmark & \xmark & \cmark & 26.29\\ 
\cmark & \cmark & \cmark & \textbf{26.48}\\ 
% \cmark & \cmark & \xmark & \\ 
% \cmark & \cmark & \cmark & 24.59\\ 
\bottomrule
\label{table:abl-np}
\end{tabular}
}
\vspace{-8mm}
\end{table}

% \noindent 
\noindent{\textbf{Importance of Geometric Bases.}}
%\str{The table seems a bit redundant, similar numbers are in the previous table. Maybe keep the new numbers only? Or merge somehow the tables?}
We also explore the effectiveness of the proposed geometric bases. As shown in Table~\ref{table:abl-np} (rows 1 and 5), with the geometric bases, \method{} performs clearly better. This indicates the importance of the 3D structure information modeled in the geometric bases, which provide specific inferences of the INR function in different spatial levels. Moreover, the bases perform well without hierarchical latent variables, demonstrating their ability to construct 3D information and reduce misalignment between 2D and 3D spaces.


% provide  effectively encodes modulates inputs, making them context-specific. Consequently, even with a fully shared MLP, the model can produce reliable estimations.

% \wy{Need to figure out how to structure two tabless}
%The reason is that the input is re-represented by the Gaussian basis, which indicates the effectiveness of our Gaussian basis. Ho
%\str{What do you mean here by re-represented?}
%For the experiment without the Gaussian basis, we simply use the coordinate embedding with Fourier features and an MLP to obtain the representation of each location. \str{What are coordinate embeddings? I think you must again make sure the wording, terminology and styling is consistent.}
%Then, the global and location variables are obtained by aggregating this representation. The experiment shows that the performance significantly drops without the help of the Gaussian basis. 

%\noindent {\textbf{Ablation study on NP hierarchical maybe? }}

% \noindent 


% 
% the performance is close to the best one. 

% \begin{table}[h]
% \centering
% \caption{Ablation study of the number of Gaussians basis on image regression.}
% \label{your-label}
% \begin{tabular}{lccc}
% \toprule
% \# Basis & 49 & 169 & 484 \\ \midrule
% -     & 28.59  & 33.74   &  44.24  \\ \bottomrule
% \label{table:num-gaussian}
% \end{tabular}
% \end{table}



% \begin{table}[h]
% \centering
% \caption{Ablation study of the number of Gaussians basis on NeRF.}
% \label{your-label}
% \begin{tabular}{lccc}
% \toprule
% \# Basis & 100 & 250 & 441 \\ \midrule
% -     &   & 24.59   &    \\ \bottomrule
% \label{table:num-gaussian-3d}
% \end{tabular}
% \end{table}

% \noindent{\textbf{Uncertainty Visualization}.} 
% As a probabilistic framework, our method can provide uncertainty estimation. To obtain the uncertainty map, we sample ten times from the predicted prior distribution to generate corresponding images and then use the variance map to represent the uncertainty. As shown in Fig.~\ref{fig:uncertainty-visual}, high uncertainty is concentrated around the edges, which is expected, as capturing detailed, sharp changes at the edges is more challenging for the model.

% \begin{figure}[t!]
%   \centering
%   \includegraphics[width=0.99\textwidth]{ICLR2025/Figures/uncertainty.pdf} % Adjust the size and filename as needed
%   \vspace{-3mm}
%   \caption{\textbf{Uncertainty Map of the predictions.} Edges of objects have higher uncertainty since it is more challenging for the model to capture the detailed, sharp changes at the edges.}
%   \label{fig:uncertainty-visual}
%   \vspace{-3mm}
% \end{figure}



% \begin{figure}[t]
%     \centering
    % \begin{minipage}[b]{0.45\textwidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{Figures/image_with_heatmap_2.png}
    %     %\caption{Figure 1}
    %     \label{fig:figure1}
    % \end{minipage}
    % \hfill
    % \begin{minipage}[b]{0.45\textwidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{Figures/image_with_heatmap_9.png}
    %     %\caption{Figure 2}
    %     \label{fig:figure2}
    % \end{minipage}
    % \vskip\baselineskip
%     \begin{minipage}[b]{0.45\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{Figures/image_with_heatmap_14.png}
%         %\caption{Figure 3}
%         \label{fig:figure3}
%     \end{minipage}
%     \hfill
%     \begin{minipage}[b]{0.45\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{Figures/image_with_heatmap_16}
%         %\caption{Figure 4}
%         \label{fig:figure4}
%     \end{minipage}
%     \caption{\textbf{Uncertainty Map of the predictions.} Edges of objects have higher uncertainty since it is more challenging for the model to capture the detailed, sharp changes at the edges.}
%     \label{fig:uncertainty-visual}
%     \vspace{-4mm}
% \end{figure}



==> Sections/intro-bk.tex <==

%1. what's NeRF

Neural Fields (NeFs) and Implicit Neural Representations (INRs)~\citep{sitzmann2020implicit,tancik2020fourier} have recently gained popularity for their ability to learn continuous, compact, and efficient representations of continuous signals, especially for 3D settings~\citep{park2019deepsdf,mildenhall2021nerf,mescheder2019occupancy,chen2022tensorf}. Building on NeFs, neural radiance fields (NeRFs)~\citep{mildenhall2021nerf,barron2021mip} model 3D scene representation as a mapping from 3D coordinates and view directions to color and density values. By integrating these values along camera rays, NeRFs can render photorealistic images of scenes from novel viewpoints. 
Although NeRFs achieve good reconstruction performance, they must be overfitted to each 3D object or scene, resulting in poor generalization to new 3D scenes with few context images.

% Thus, fast adaptation of NeRF representations for new 3D scences is still unexplored 
% Thus, one of the main challenges of NeRFs is to improve their generalization for novel 3D scenes.

% popular for representing data as neural functions, mapping continuous coordinates to signals.
% For instance, 3D scene representations~\cite{park2019deepsdf,mildenhall2021nerf,mescheder2019occupancy,chen2022tensorf} favor INRs due to their continuous, compact, and efficient data representation properties.
% However, characterizing a signal by neural network parameters often requires retraining the network on individual data samples, which is computationally expensive.
% Therefore, models must quickly adapt to new signals from partial observations without extensive fine-tuning.

% \zx{This paragraph is a bit long.}

%Despite the need of fast generalization to the new scene for real-time rendering, 
%\str{I am not sure I follow the logic of this paragraph. We are mixing metalearning, probabilistic learning, 3D and 2D partial obersbation, global and local. What exactly is our point?}
In this paper, we focus on radiance field generalization and fast adaptation of the INR function for novel 3D scenes using only a few context image views. Previous works on INR generalization have approached the problem by gradient-based meta-learning~\citep{tancik2021learned} to adapt to new scenes with a few optimization steps~\citep{tancik2021learned,papa2023train}, 
%\str{Add the CVPR reference for Samuele}
modulating shared MLPs through HyperNets~\citep{chen2022transformers,mehta2021modulated,dupont2022data,kim2023generalizable}, or directly predicting the parameters of scene-specific MLPs~\citep{dupont2021generative,erkocc2023hyperdiffusion}. However, the deterministic nature of these methods cannot account for the uncertainty of scenes or INR functions when only few partial observations are available. This is unrealistic since there can be different interpretations of limited observations. 

To account for uncertainty induced by few available context images, probabilistic INR functions for NeRF \citep{gu2023generalizable, guo2023versatile, kosiorek2021nerf} have also been recently explored. VNP~\citep{guo2023versatile} and PONP~\citep{gu2023generalizable} infer the INR function using Neural Processes (NPs)~\citep{bruinsma2023autoregressive, garnelo2018neural, wang2020doubly, shen2024episodic}, a probabilistic meta-learning method that models functional distributions conditioned on partial signal observations.
\str{I think this is not a very strong way of putting it, sounds too niche. I would rather say that NeRF is basically a mapping from a collection of 2D input domain to 3D output domain. These methods focus on the 3D only, that is the output, without account for the fact that this uncertainty should also be directly grounded in the 2D input domain. To make it sound more fundamental (the way it already is).}
These probabilistic methods, however, only approximate the INR functions in 3D space, neglecting the interaction between 3D functions and 2D observations. 
% Radiance fields model 3D relationships, but the context is just 2D posed images. The inherent information misalignment between the radiance field function and context images could hinder these models' generalization.
Since the radiance fields model relationships in 3D space, while the only available context observations are 2D images, there is an information misalignment between contexts and functions in radiance field generalization.


%\str{What is probabilize? There is no such word.}
% However, these methods only probabilize the INR functions in the 3D space, neglecting the interaction between 3D functions and 2D partial observations. 
% In contrast, some other methods model in probabilistic perceptives. 
% NeRF-VAE~\cite{kosiorek2021nerf} learns a distribution over radiance fields conditioning on a latent scene representation. 
%Some other works~\cite{} utilize GAN~\cite{goodfellow2020generative} to implicitly learn the distribution of functions. 

% Therefore, despite being probabilistic, the function inferred from 2D observation partials is suboptimal due to the information loss from 2D to 3D spaces.
% Neural processes (NP) is also a meta-learning method, but in a probabilistic manner~\cite{bruinsma2023autoregressive}, which aims to model the distribution of functions given partial observations. In this work, we aim to model the distribution of implicit functions, which aligns with the formulation of NPs. 

%\str{Can we make clear what are the contributions, in short?}
\str{Unclear (in the first sentence) why the solution is specific to the problem we highlighted in the previous paragraph (the discrepancy between 2D and 3D)? It becomes sort of clear in the 2) ..., but it has to be more explicit and direct. What exactly is the relation between 2D and 3D geometry, and how do we make it possible to model this? This has to be in the first sentence, and also in the explanation later on. 'Observations in 2D space with 3D prior structures' sounds a bit vague, not as explicit as it can be. Also, 1, 2, 3, feel a bit disconnected. Is 3 just a random add on that is orthogonal to 1 and 2? Until now, we never talked about the multi-scale nature of geometric structures in the world. I would say that this a key point, if others don't really account for this. Overall, this paragraph needs to be rewritten.}
To efficiently adapt to new signals with few observations, 
we propose probabilistic radiance field generalization with Geometric Neural Processes (\name{}). 
Our contributions can be summarized as follows: 
\textit{1) Probabilistic NeRF generalization framework.}  We cast radiance field generalization as a probabilistic modeling problem. By doing so, we can amortize the probabilistic model over multiple objects with few views, facilitating the learning and generalization of NeRF functions.
% can accelerate the learning and generalize by amortizing the probabilistic model over multiple objects
% For NeRF generalization, we accelerate the learning and generalize by amortizing the probabilistic model over multiple objects and then obtaining per-object reconstructions by conditioning on context sets $\{{\widetilde {\bf{X}}}_C, {\widetilde {\bf{Y}}}_C\}$.
% The probabilistic model contains an INR function in 3D space and the transition between 2D and 3D variables (ray sampling and integration). This enables to design stochastic processes to model the INR function in 3D by considering the probabilistic interaction between 2D and 3D variables.
\textit{2) Geometric bases.} To eliminate the 
potential information misalignment, we design geometric bases by encoding observations in 2D space with 3D prior structures. Thus, the geometric bases can aggregate locality information to each 3D point, improving the exploration of high-frequency details.
\textit{3) Geometric neural processes with hierarchical latent variables.}
Based on the geometric bases, we develop geometric neural processes to capture the uncertainty in the latent NeRF function space.
Specifically, we introduce hierarchical latent variables to modulate the INR function at multiple spatial levels, yielding better generalization on new scenes and new views.
% incorporates prior structure information with  into the inference of the INR function distribution. 
% The hierarchical latent variables enable modulating the INR function at multiple spatial levels, thus improving the generalization of INR functions.
Experiments on novel view synthesis of ShapeNet objects and real-world DTU scenes demonstrate the effectiveness of the proposed method on 3D radiance field generalization. Nevertheless, the proposed method can seamlessly apply to INR generalization in 2D signals (images). %settings.

% Specifically, we train an attention-based neural network to construct a set of geometric bases from the 2D context observations. 
% Consisting of 3D Gaussians, the geometric bases provide structure information and representations of the 3D scenes, which are utilized to infer the function distribution in 3D. 
% Furthermore, with the geometric bases, we introduce hierarchical latent variables in both object and ray levels to infer the predictive function. 
% By fully utilizing the 3D information provided by the geometric bases, the latent variables specialize information of different spatial levels, achieving both object-specific and ray-specific INR functions for generalization on limited contexts.


% ++++++++++++++++++ editing

% Despite the previous effort on modeling probabilistic INR, they ignore the structure information in the space and only focus on the global object-level latent variable or modulation. 
% %However, such works ignore the information loss from the 2D context observation to the 3D space \wy{sampling issues, maybe refer learn to sample paper} and lack structure information. 
% %Moreover, the hierarchical neural process in VNP is sequential, not exploring the structure information. 
% % However, such methods ignore the local information, resulting in missing the high-frequency details of objects. 
% The structure information is a proxy between the ``generality'' and “specialization”~\cite{cong2023enhancing,bauer2023spatial}. To achieve generality, the model should be able to capture the shared context, which is the global object level. On the other hand, to have high-fidelity rendering results, the model should be able to infer the sample-specific or region-specific information, e.g. specialized self-similar appearance patterns, which is at the local level. 
% In this work, we propose to use hierarchical neural processes (HNP)~\cite{wang2022learning,wang2020doubly,shen2024episodic} to model the distribution of functions, which allows us to explicitly introduce a global and local variable to incorporate the structure information globally and locally. 
% We found that our local variable suits the neural radiance field (NeRF) framework well. Hence,
% to better demonstrate our local variable, we illustrate our method on neural radiance field generalization.
% However, our method is also applicable to other INRs, such as image regression and image completion, as shown in our experiments. 


% In an NPs setting, the context set is given to infer a function for the target set, which models a conditional distribution. For neural radiance fields (NeRF), the context set is the few-view images with the corresponding camera rays. 
% However, the NeRF function we aim to approximate is inherited in 3D space. There exists a gap between the context information and the NeRF function
% %, which is commonly ignored in previous INR generalization literature 
% due to the sampling and integration\cite{martin2021nerf,arandjelovic2021nerf,fang2021neusample,lindell2021autoint,neff2021donerf} from the camera ray to the projected 2D image pixels. \wy{discussion: these papers all about how to improve sampling to speed up the Monte Carlo for efficient training.} This may cause information loss between 2D context and 3D function.
% %inconsistency in formulation. 
% %For instance, 3D points are sampled along the rays~\cite{martin2021nerf}, which may affect the quality of integrating information along camera rays to render the corresponding pixels~\cite{arandjelovic2021nerf}. 
% Instead of directly building the conditional distribution on observed camera rays and projected 2D images, we derive our function distribution fully on the 3D space based on a set of geometric Gaussian basis spanned in space, 
% %Specifically, we choose to use the Gaussian basis due to its continuous property
% which is favored by previous 3D reconstruction methods~\cite{genova2020local,chen2023neurbf,kerbl20233d}. The geometric Gaussian basis is able to reflect the shape of objects (global structure) and aggregate the locality information~\cite{chen2023neurbf,chen2022tensorf} into arbitrary 3D locations in a continuous way.  
% Finally, we provide evidence of a lower bound to train the model. Our approach enables neural radiance field generalization in a single feedforward pass, without fine-tuning. Our contributions can be summarized as follows:
% \begin{enumerate}
%     \item We propose a new probabilistic formulation for NeRF generalization based on hierarchical neural processes, which is also applicable to general INR generalization.
%     \item We propose to infer a set of posterior geometric bases to embed the structure information globally and locally. 
% \end{enumerate}










%RBF kernels have been explored in previous NeRF research
%, as well as other 3D scene reconstruction techniques, like Gaussian Splatting~\cite{kerbl20233d} which assumes the space is composed of a set of Gaussians. 

%To address the above-mentioned issues, we introduce a set of geometry basis spanned in space to provide structure information. 
%In 3D NeRF, this can also eliminate the information loss by directly inferring the continuous 3D space basis from the 2D context information. Then, we contribute to a neural processes formulation of NeRF, based on which we perform hierarchical NP. The hierarchical NP consists of a global variable that models the scene information and a local variable that models the ray-wise or location-wise information. Finally, we provide evidence of a lower bound to train the model. Our approach enables neural radiance field generalization in a single feedforward pass, without fine-tuning. 


%


%-------------------------------------------------

% comments of why using basis:
% 1. For modeling the local neural features (check how this local neural features help?). because of the difficulty
% in representing high-frequency details due to the inductive
% bias [5, 70] of MLPs. To tackle this problem, local neural fields have been proposed and widely adopted. 

% 2. 3D Gaussians as a flexible and expressive scene representation

% 2. flexible kernel position and shape, which have higher spatial adaptivity and can more closely fit target signals

% 3. challenges of current Radiance Field Generalization methods(do not consider uncertainty, fine-tuning, time-consuming, balabala),
% why we use NP

% 4. What we do in our method (our contributions) (model the problem in a probabilistic framework to infer the function for Radiance Field Generalization in a single feedforward pass, without fine-tuning; propose geometric basis to solve the information gap between 2D context and 3D target function; hierarchical neural processes/modulation for XXX)


% The idea of using Geometry bases origins from the previous NeRF works~\cite{chen2022tensorf,muller2022instant} which use either gird regular point latent representation or RBF kernels in the space, to store the 3D scene geometry and semantic information, as well as the Gaussian Splatting~\cite{kerbl20233d} which assumes the space is composed of a set of Gaussians. 


%GENERALIZATION IN DIFFUSION MODELS ARISES FROM GEOMETRY-ADAPTIVE HARMONIC REPRESENTATIONS shows the geometry prior basis connect to our motivation.

% Keypoint: 

% 1. We want to model the distribution of functions to achieve implicit neural field generalization, which is suitable for Neural Processes. 

% 2. The context information has an information gap with the 3D Radiance Field. Previous generalization work, including VNP~\cite{guo2023versatile} ignores this. This motivates us to introduce a set of Gaussian basis to encode the geometry information in the scene. Also, by doing so, we are able to connect NP and NeRF generalization more tightly. 

% 3. The Gaussian basis with radial basis function provides a continuous way of representing each spatial location. 
